TURF: A Two-factor, Universal, Robust, Fast Distribution Learning Algorithm

Approximating distributions from their samples is a canonical statistical-learning problem. One of its most powerful and successful modalities approximates every distribution to an $\ell_1$ distance essentially at most a constant times larger than its closest $t$-piece degree-$d$ polynomial, where $t\ge1$ and $d\ge0$. Letting $c_{t,d}$ denote the smallest such factor, clearly $c_{1,0}=1$, and it can be shown that $c_{t,d}\ge 2$ for all other $t$ and $d$. Yet current computationally efficient algorithms show only $c_{t,1}\le 2.25$ and the bound rises quickly to $c_{t,d}\le 3$ for $d\ge 9$. We derive a near-linear-time and essentially sample-optimal estimator that establishes $c_{t,d}=2$ for all $(t,d)\ne(1,0)$. Additionally, for many practical distributions, the lowest approximation distance is achieved by polynomials with vastly varying number of pieces. We provide a method that estimates this number near-optimally, hence helps approach the best possible approximation. Experiments combining the two techniques confirm improved performance over existing methodologies.

==> appenconc.tex <==
\section{Intervals and Partitions}
%\begin{Lemma}
%For any $ 0\le a<b\le n $, $\epsilon\ge 0$,
%\ignore{-.5em}
%\[\Pr[|\intp_{a,b}-\hatp_{a,b}|\ge \epsilon\sqrt{\hatp_{a,b}}]
%\le 
%e^{-(n-1)\frac{\epsilon^2}{2}}
%+e^{-(n-1)\frac{\epsilon^2
%\hatp_{a,b}}{2(\hatp_{a,b}+\epsilon\sqrt{\hatp_{a,b}})}}.
%\ignore{-.75em}\]
%\end{Lemma}
\subsection{Proof of Lemma~\ref{lem:singleconc}}
\begin{Proof}
For simplicity, let 
$$ X\ed \intp_{a,b} ,\ \ p \ed  \hatp_{a,b}$$ so that
$ X = \intp_{a,b}\sim \Beta(n \hatp_{a,b},
n(1-\hatp_{a,b})) = \Beta(np,n(1-p))$.
For any $x,y\in\reals^+$, let
$\text{B}(x,y)=\Gamma(x)\Gamma(y)/\Gamma(x+y)$
denote the beta function and let
$a,b>0$ and $x\in[0,1]$, 
$$I_x(a,b) \ed \int_{0}^{x} 
\frac{z^{a-1}(1-z)^{b-1}}{\text{B}(a,b)} dz$$
be the incomplete beta function. Then,
\begin{align*}
\Pr[X\le p-\epsilon\sqrt{p}]&\overset{(a)}{=} 
I_{p-\epsilon\sqrt{p}}(np,n(1-p))\\
&\overset{(b)}{=}\sum_{i=np}^{n-1} {n-1\choose i} 
(p-\epsilon\sqrt{p})^i(1-p+\epsilon\sqrt{p})^{n-1-i}\\
&\overset{(c)}{\le} e^{-(n-1)D(p||p-\epsilon\sqrt{p})}\\
&\overset{(d)}{\le} e^{-(n-1)\frac{\epsilon^2}{2}},
\end{align*}
where $(a)$ follows by definition,
$(b)$ follows by the property of 
incomplete beta function~\cite{incompnist}, 
$(c)$ follows from the Chernoff bound 
applied to the right tail of a $\text{Binom}(n,p-\epsilon\sqrt{p})$ 
random variable, and $ (d) $ follows since 
$ D(x||y)\le (x-y)^2/\max\{x,y\} $. Similarly,
\begin{align*}
\Pr[X\ge p+\epsilon\sqrt{p}]
&\overset{(a)}{=}1-I_{(p+\epsilon\sqrt{p})}(np,n(1-p))\\
&\overset{(b)}{=}1-
\sum_{i=np}^{n-1} {n-1\choose i} 
(p+\epsilon\sqrt{p})^i(1-p-\epsilon\sqrt{p})^{n-1-i}\\
&\le\sum_{i=0}^{np} {n-1\choose i} 
(p+\epsilon\sqrt{p})^i(1-p-\epsilon\sqrt{p})^{n-1-i}\\
&\overset{(c)}{\le} e^{-(n-1)D(p||p+\epsilon\sqrt{p})}\\
&\overset{(d)}{\le} e^{-(n-1)\frac{\epsilon^2 p}{2(p+\epsilon\sqrt{p})}},
\end{align*}
where $(a)$ follows by definition,
$(b)$ follows by the property of 
incomplete beta function~\cite{incompnist}, and
$(c)$ follows from Chernoff bound applied to the left tail of a
$\text{Binom}(n,p+\epsilon\sqrt{p})$ random variable, and 
$ (d) $ follows since $ D(x||y)\le (x-y)^2/\max\{x,y\} $.
\end{Proof}

\subsection{Proof of Lemma~\ref{lem:multconc}}
%\begin{Lemma}
%\label{lem:multconc}
%For any $n\ge 128$,
%\[
%P[\cQ_{\epsilon}]\ge 1- ne^{-n\epsilon^2/5}
%\]
%\end{Lemma}
\begin{Proof}
From using the union bound, we have
\begin{align*}
1-\Pr[\cQ_{\epsilon}]&=
\Pr\left[\exists 0\le a<b\le n :
|\intp_{a,b}-\hatp_{a,b}|\ge
\epsilon \sqrt{\hatp_{a,b}}\right]\\
&\le \sum_{0\le a<b\le n }
\Pr\left[
|\intp_{a,b}-\hatp_{a,b}|\ge
\epsilon\sqrt{\hatp_{a,b}}\right]\\
&\overset{(a)}{\le} \sum_{0\le a<b\le n }
\left(e^{\frac{-(n-1)\epsilon^2}{2}}
+e^{\frac{-(n-1)\epsilon^2 \hatp_{a,b}}
{2(\hatp_{a,b}+\epsilon\sqrt{\hatp_{a,b}})}}\right)\\
&\overset{(b)}{=}\frac{n(n+1)}{2}
\left(e^{\frac{-(n-1)\epsilon^2}{2}}
+e^{\frac{-(n-1)\epsilon^2 \hatp_{a,b}}
{2(\hatp_{a,b}+\epsilon\sqrt{\hatp_{a,b}})}}\right)\\
&\overset{(c)}{\le} \frac{n(n+1)}{2}
\left(e^{\frac{-(n-1)\epsilon^2}{2}}
+e^{-\frac{(n-1)\epsilon^2
}{2(1+\epsilon\sqrt{n})}}\right),
%for camera ready, need to change main algo 
%so that the mass in light bins is bounded by
%$\sqrt{n}/\delta$
%to $\epsilon\ge 1/$\sqrt{n}$.
%\\
%&\overset{(d)}{\le}
%\frac{n(n+1)}{2}
%\left(e^{\frac{-(n-1)\epsilon}{2\sqrt{n}}}
%+e^{-\frac{(n-1)\epsilon
%}{4\sqrt{n}}}\right)\\
%&\overset{}{\le}
%\frac{n(n+1)}{2} 
%\cdot 2e^{-\frac{(n-1)\epsilon}{4\sqrt{n}}},
\end{align*}
where $(a)$ follows from Lemma~\ref{lem:singleconc},
$(b)$ follows since $ |0\le a<b\le n| = 
\binom{n+1}{2} $, and $ (c) $ follows since $q_{a,b}\ge 1/n $. 
%and $ (d) $ follows since $ \epsilon \ge 1/\sqrt{n}$.
%Noting that $ n\ge 128$ completes proof for the ranges
%of $ \epsilon $ we consider.
\end{Proof}

==> appenintro.tex <==
\section{Main Results}
\begin{Theorem}
\label{thm:polyblack}
Given $ X^{n-1}\sim f $, for some $ n\ge 128 $,
degree $  d$, and an interval $ I $ with 
$ \hatp_I n $ samples, $ \EQ $ 
takes $ \cO(d^\tau+\hatp_I n) $ time,
and outputs $ \hatf_{I, \EQ}\in \cP_d $
such that w.p. $ \ge 1-\delta $,
\begin{align*}
\nonumber
\loneint{I}{\hatf_{I, \EQ}-f}
&\le (r_d+1)\cdot \inf_{\poly \in \cP_d} \loneint{I}{\poly - f }\\
%\label{eqn:blackbox}
&\phantom{\le}
+r_d \cdot \sqrt{\frac{5(d+1)\hatp_I\log \frac{n}{\delta}}{n}},
\end{align*}
where $ \loneint{I}{.} $ is the $ \ell_1 $ distance
evaluated on $ I $, $\tau < 2.4$ is the matrix 
inversion exponent, $ r_d $ is a fundamental constant
whose values are $ r_0 = 1, r_1 = 1.25, r_2 \approx 1.42 , r_3 \approx
1.55 $, $ r_4\le 1.675 $, $ r_5\le 1.774 $, 
$ r_6\le 1.857 $, $ r_7\le 1.930 $, $ r_8\le 1.999$
for $ 4\le d \le 8 $.
\end{Theorem}
\begin{Proof}
For a given $ d $, $ \EQ $ outputs 
$\hatf_{I, \mathrm{EQ}} = \hatf_{I,\barn_{d}}$
given by the corresponding $ \barn_{d} \in \cN_d $ in 
Lemma~\ref{lem:optnodes}.
Using Lemma~\ref{lem:ratioconst} completes the proof.
\end{Proof}
%
\begin{Theorem}
\label{thm:interhistopt}
Given $X^{n-1}\sim f$, for some $ n\ge 128 $ such 
that $ n $ is a power of $ 2 $, and parameters 
$d\le 8$, $ \alpha>2 $, $ \SURF $ takes 
$ \cO((d^{\tau}+\log n)n\log n) $ time,
and outputs $ \hatf_{\text{SURF}}$
such that w.p. $ \ge 1-\delta $,
\ignore{-.25em} 
\begin{align*}
&\lone{\hatf_{\text{SURF}}-f}\\
&\le
\min_{\barI\in \Delta_{\reals}}\sum_{I \in \barI} 
\left(
\frac{(r_d+1)\cdot \alpha}{\alpha-2}\cdot 
\inf_{\poly \in \cP_d} \loneint{I}{\poly - f }\right.\\
&\phantom{\le\min_{\barI\in \Delta_{\barI}}}
\left.\ +\frac{r_d\cdot (\alpha\sqrt2+\sqrt{2}-1)}{(\sqrt{2}-1)^2}
\sqrt{\frac{5(d+1) \hatp_I \log \frac{n}{\delta}}{n}}\right),
\end{align*}
where $\Delta_{\reals}$ is the collection of all 
partitions of $ \reals $ whose intervals
start and end at a sample point, 
$ |\barI| $ is the number of intervals in $ \barI \in \Delta_{\reals}$,
$ \hatp_I\cdot n $ is the number of samples in interval $ I \in \barI$,
$ \tau < 2.4 $ is the matrix inversion exponent, 
and $ r_d>0$ is the constant in Theorem~\ref{thm:polyblack}.
\end{Theorem}
\begin{Proof}
The claim follows under event $ \cQ_{\delta} $ upon 
using Lemma~\ref{lem:binarycomp} 
on top of Lemma~\ref{lem:master}. 
Finally, for $n\ge 128$, $ \cQ_{\delta} $ holds with 
probability $ \ge 1-\delta $ from Lemma~\ref{lem:multconc}.
\end{Proof}
%
\begin{Corollary}
\label{cor:interhistopt}
Running $ \SURF$ with $ n\ge 128,\alpha>2, d\le 8$,
\begin{align*}
&\EE\lone{\hatf_{\SURF}-f}\\
&\le \min_{t\ge 0} \left( 
(r_d+1)\cdot \mathrm{OPT}_{\cP_{t,d}}(f)+
\tilde{\cO}\left( \sqrt{\frac{t\cdot (d+1)}{n}}\right)
\right).
\end{align*}
\end{Corollary}




==> appenpoly.tex <==
\section{The Interpolation Routine}
\subsection{Proof of Lemma~\ref{lem:ratioconst}}
%\begin{Lemma}
%\label{lem:ratioconst}
%For interval $ I=[0,1]$ with empirical probability 
%$ \hatp_I $, any $ \barn_d\in\cN_d $, 
%and $ \epsilon>0 $, the estimate $ \hatf_{\barn_d} $~\eqref{eqn:areamatch} is such that
%under event $ \cQ_{\epsilon} $,
%\begin{align*}
%\lone{\hatf_{\barn_d}-f} 
%&\le 
%\left(1+r_d(\barn_d)\right)
%\inf_{\poly \in \cP_d}\lone{\poly-f} \\
%&\phantom{\le}
%+r_d(\barn_d) \epsilon \sqrt{(d+1)\hatp_I}.
%\end{align*}
%\end{Lemma}
\begin{Proof}
For a partition $ \bar{I}$ of $ I=[0,1] $,
and integrable functions $ g_1, g_2 $, define the distance 
\begin{equation}
\label{eqn:ddistance}
d_{\bar{I}} (g_1,g_2) 
\ed \sum_{J\in \bar{I}} \Big|\int_J g_1 - \int_J g_2\Big|.
\end{equation}
In words, $ d_{\bar{I}} (g_1,g_2)  $ is the sum of
absolute differences between measures under
$ g_1 $ and $ g_2 $ across all intervals in $ \bar{I} $.
For any $ \poly \in \cP_d $,
\begin{align*}
\loneint{I}{\hatf_{\barn_d}-f} &\le \loneint{I}{\poly-f} + 
\loneint{I}{\hatf_{\barn_d}-\poly} \\
&\overset{(a)}{\le} \loneint{I}{\poly-f} + r_d(\barn_d)d_{\bar{I}_{\barn_d}}(\poly,\hatf_{\barn_d})\\
&\overset{(b)}{\le} \loneint{I}{\poly-f} + 
r_d(\barn_d)\left(d_{\bar{I}_{\barn_d}}(\poly,f) + d_{\bar{I}_{\barn_d}}(f,\hatf_{\barn_d})\right)\\
&\overset{(c)}{\le} \left(1+r_d(\barn_d)\right)\loneint{I}{\poly-f}+ 
r_d(\barn_d)d_{\bar{I}_{\barn_d}}(f,\hatf_{\barn_d})\\
&\overset{(d)}{\le} \left(1+r_d(\barn_d)\right)\loneint{I}{\poly-f} + 
r_d(\barn_d)\sum_{J\in \barI_{\barn_d}}
|\intp_J-\hatp_J|\\
&\overset{(e)}{\le} \left(1+r_d(\barn_d)\right)\loneint{I}{\poly-f} + 
r_d(\barn_d)\sum_{J\in \barI_{\barn_d}}
\epsilon\sqrt{ \hatp_J }\\
&\overset{(f)}{\le} \left(1+r_d(\barn_d)\right)\loneint{I}{\poly-f} + 
r_d(\barn_d)
\epsilon\sqrt{\hatp_I (d+1)},
\end{align*}
where $ (a) $ follows since $ (\poly-\hatf_{I,\barn_d})\in \cP_d $,
and from definitions of the ratio $ r_d(\barn_d) $ 
in Equation~\eqref{eqn:polyrat},
$ (b) $ follows since the $ d_{\barI} $-distance 
satisfies the triangle inequality,
$ (c) $ follows since the $ \ell_1 $ distance upper
bounds $ d_{\barI}-$distance, 
$ (d) $ follows since $ \hatf_{\barn_d} $,
by definition, is the polynomial such that
$ \int_J \hatf_{\barn_d} = \hatp_{J}$ $ \forall J\in \barI_{\barn_{d}} $, and 
the interval probability $ \intp_{J}\ed \int_{J} f $,
$ (e) $ follows under event $ \cQ_{\epsilon}$, and
$ (f) $ follows since by the concavity of 
$ \sqrt{x} $ for $ x\ge 0 $, the sum 
$ \sum_{J\in \barI_{\barn_d}} \sqrt{ \hatp_J } $ is
maximized if for each $ J\in \barI_{\barn_{d}} $, 
$\hatp_J = (\sum_{J\in 
\barI_{\barn_d}} \hatp_J)/|\barI_{\barn_d}|= \hatp_{I}/(d+1)$.
\end{Proof}

\subsection{Proof of Lemma~\ref{lem:zeroish}}
%\begin{Lemma}
%\label{lem:zeroish}
%For any degree-$d$ and $ \barn_d\in\cN_d $,
%\[r_d(\barn_d)=\sup_{\poly\in\cP_d}r(\barn_d,h)
%=\max_{\poly\in\cP_{\barn_d}}r(\barn_d,h).\]
%\end{Lemma}
\begin{Proof}
Fix $ \poly\in \cP_{d} $. Let $(\beta_1,\upto ,\beta_{d_0}) $ be
the roots of $ \poly$ in $ [0,1] $ for some 
$ \beta_1\le \upto \le \beta_{d_{0}}, 0\le d_{0}\le d $.
Let $ \beta_{0}\ed 0, \beta_{d_{0}+1}\ed 1 $.
Then notice that 
\[
\int_{0}^{1} |h|  =\sum_{i=1}^{d_0+1}\Big |\int_{\beta_{i-1}}^{\beta_{i}}  h\Big |
\overset{(a)}{\le} \sup_{\barm_d\in \cN_d } 
\sum_{i=1}^{d+1}\Big |\int_{m_{i-1}}^{m_{i}}  h\Big |
=\sup_{\barm_d\in \cN_d } \max_{\bar{s}\in \{0,1\}^{d+1} }
\sum_{i=1}^{d+1}(-1)^{s_i}\int_{m_{i-1}}^{m_{i}}  h
\overset{(b)}{\le}\int_{0}^{1} |h|,
\]
where $ (a) $ follows since on padding $ d-d_{0} $ zeros,
$ (0,\cdots, 0, \beta_{0}\upto \beta_{d+1})\in \cN_d $.
Thus $ (b) $ is, in fact, an equality, implying
%let $H \in \cP_{d+1}$ denote
%its integral, where the constant of integration is fixed
%using $H(0)=0$. Let $\sum_{i=1}^{d+1}  c_i x^{i} \ed H(x)$. Then
\begin{align*}
r_{d}(\barn_d) 
=\sup_{\poly\in \cP_d}r(\barn_{d},\poly)
&= \sup_{\poly\in \cP_d}
\frac{\int_{0}^1|h|}{\sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}
\poly|}\\
&=
\sup_{\poly\in \cP_d}
\frac{\sup_{\barm_d\in \cN_d}\max_{\bar{s}\in \{0,1\}^{d+1} }
\sum_{i=1}^{d+1}(-1)^{s_i}\int_{m_{i-1}}^{m_i}h}
{\sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}h|}\\
&=\sup_{\barm_d\in \cN_d}\max_{\bar{s}\in \{0,1\}^{d+1} }
\sup_{\poly\in \cP_d}
\frac{\sum_{i=1}^{d+1}(-1)^{s_i}\int_{m_{i-1}}^{m_i}h}
{\sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}h|}.
\end{align*}
Denote $ h = \sum_{i=1}^{d+1} c_{i}\cdot  x^{i-1}  $
and let $ \bar{c}\ed(c_1\upto c_{d+1}) $.
Notice that since $ r(\barn_{d}, \poly)\ge 1 $
for any $ \poly \in \cP_d $, and since $ r_d(\barn_{d}, 0)\ed 1 $,
WLOG assume $ \poly \neq 0 $ or
$ \bar{c}\neq \bar{0}\ed (0\upto 0) $.
By linearity of the integral of $\poly $ in $ \bar{c}$, recast $ r_{d}(\barn_{d}) $ into
\[
r_{d}(\barn_{d}) = 
\sup_{\barm_{d}\in {\cN_{d}}}\max_{\bar{s}\in \{0,1\}^{d+1} }
\sup_{\bar{c}\in \reals^{d+1}\setminus\{\bar{0}\}}
\frac{\sum_{i=1}^{d+1}c_i\mu_{i}}
{\sum_{i=1}^{d+1}|\sum_{j=1}^{d+1}c_j\lambda_{i,j}|},
\]
where for any $ i, j \in \{1\upto d+1\} $,
$ \mu_{i}\in \reals $ is a function of $ \barm_d,\bar{s} $ and
$\lambda_{i,j} \in \reals$ is a function of $\barn_d $.
Observe that $ \barn_{d} $ is given, and additionally 
fix $ \barm_{d}\in \cN_{d} $, $ \bar{s}\in \{0,1\}^{d+1} $.
Since the objective function here is a ratio whose denominator is 
positive (since $ h\neq 0 $), WLOG set the numerator 
to $ 1 $ via the constraint $\sum_{i=1}^{d+1}c_i\mu_{i}=1 $ 
and convert it to a linear program as:
\[
\max
\frac{1}{\sum_{i=1}^{d+1} v_i } : \bar{c}, \bar{v} \in \reals^{d+1}, \
\ v_i\ge \sum_{j=1}^{d+1}c_j\lambda_{i,j}, \
v_i \ge -\sum_{j=1}^{d+1}c_j\lambda_{i,j},
\sum_{i=1}^{d+1} c_i\mu_i =1,
\]
where $ \bar{v}\ed (v_1\upto v_{d+1})  $.
Observe that these constraints give rise to a 
bounded region, and since this is a linear program, 
there exists a solution at some corner point 
involving at least $ 2\cdot (d+1) $ equalities, 
one for each variable.
In any such solution, since the equality:
$ \sum_{i=1}^{d+1} c_i \mu_i =1 $ is always active,
at least $ 2\cdot (d+1) - 1 $ of the other 
inequalities attain equality. 
Notice that for any $ i\in\{1\upto d+1\} $, 
$ v_i=0 $ if both
\[  v_i = \sum_{j=1}^{d+1}c_j\lambda_{i,j} \text{ and } 
v_i =  -\sum_{j=1}^{d+1}c_j\lambda_{i,j} \text{ hold}.\] 
Thus in this corner point solution, $ v_i \neq 0 $ for at most one $ i\in \{1\upto d+1\} $.
Let 
\[ \cD_{\barn_{d}} = \Big \{\bar{c} \in \reals^{d+1} \setminus \{\bar{0}\}:
\exists i_1\in \{1\upto d+1\}:
\forall i\neq i_1, \ |\sum_{j=1}^{d+1}c_j\lambda_{i,j}|=0\Big \}\]
This implies
\begin{align*}
r_{d}(\barn_d) 
&=\sup_{\barm_{d}\in {\cN_{d}}}\max_{\bar{s}\in \{0,1\}^{d+1} }
\sup_{\bar{c}\in \reals^{d+1}\setminus \{\bar{0}\}}
\frac{\sum_{i=1}^{d+1}c_i\mu_i}
{\sum_{i=1}^{d+1}|\sum_{j=1}^{d+1}c_j\lambda_{i,j}|}\\
&=\sup_{\barm_{d}\in {\cN_{d}}}\max_{\bar{s}\in \{0,1\}^{d+1} }
\max_{\bar{c}\in \cD_{\barn_{d}}}
\frac{\sum_{i=1}^{d+1}c_i\mu_i}
{\sum_{i=1}^{d+1}|\sum_{j=1}^{d+1}c_j\lambda_{i,j}|}\\
&=\sup_{\barm_{d}\in {\cN_{d}}}\max_{\bar{s}\in \{0,1\}^{d+1} }
\max_{\poly\in \cP_{\barn_d}}
\frac{\sum_{i=1}^{d+1}(-1)^{s_i}\int_{m_{i-1}}^{m_i}h}
{\sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}h|}\\
&= \max_{\poly\in \cP_{\barn_d}}
\sup_{\barm_{d}\in {\cN_{d}}}\max_{\bar{s}\in \{0,1\}^{d+1} }
\frac{\sum_{i=1}^{d+1}(-1)^{s_i}\int_{m_{i-1}}^{m_i}h}
{\sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}h|}\\
&= \max_{\poly\in \cP_{\barn_d}}
\frac{\int_{0}^{1}|h|}
{\sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}h|}
= \max_{\poly\in \cP_{\barn_d}} r_{d}(\barn_d,h).
\end{align*}
\end{Proof}

\subsection{Proof of Lemma~\ref{lem:optnodes}}
%\begin{Lemma}
%\label{lem:optnodes}
%For $d\le 3 $, there exists a node collection 
%$ \barn^{\star}_d $
%that achieves $ r^{\star}_d $. These,
%and their respective $ r^{\star}_d $ are given by
%\begin{center}
%\begin{tabular}{ |c|c|c| } 
%\hline
%$ d $ & $ \barn^{\star}_d $  & $r^{\star}_d$ \\ 
%\hline
%0 & $ (0,1) $ & $ 1 $ \\
%\hline
%1 & $ (0,0.5,1) $ & $ 1.25 $ \\
%\hline
%2 & $ \approx (0, 0.2599, 0.7601, 1) $ & $ \approx 1.42 $ \\ 
%\hline
%3 & $ \approx(0, 0.1548, 0.5, 0.8452, 1) $& $\approx 1.56 $\\ 
%\hline
%\end{tabular}
%\end{center}
%Denoting $\barn^{\star}_2 = (0,\alpha_0,1-\alpha_0, 1)  $, 
%and $ \barn^{\star}_3 = (0, \beta_0, 0.5, 1-\beta_0, 1) $,
%the exact values of $ \alpha _0 $, $ \beta_0 $, 
%are obtained as roots to a degree-$14$ and 
%degree-$ 69 $ polynomial that is explicitly provided.
%For degrees $ 4\le d\le 8 $, the following 
%$ \barn_d\in \cN_d$ and $ r_d(\barn_d) $ 
%provide upper bounds on $ r_d^{\star} $.
%\begin{center}
%\begin{tabular}{ |c|c|c| } 
%\hline
%$ d $ & $ \barn_d $  & $r_d(\barn_d)$ \\ 
%\hline
%4 & $ (0, 0.1015, 0.348, 0.652, 0.8985,1)$ & 
%$ < 1.675$ \\
%\hline
%5 & $ ( 0 ,   0.071 ,   0.254 ,   0.5  ,  $ &  \\ 
% & $  0.746,   0.929  ,  1) $ & $ <  1.774 $ \\ 
%\hline
%6 & $ (0,    0.053,    0.192,    0.390,    $& $ $\\ 
%& $   0.610,   0.808,   0.947,    1) $& $ < 1.857 $\\ 
%\hline
%7 & $ (0, 0.0405   , 0.149 ,  0.310,   0.5,   $ & \\
%& $  0.690,    0.851, 0.9595,    1) $ & $ < 1.930 $ \\
%\hline
%8 & $  (0,    0.032,   0.119,    0.252,    0.414,   $ &  \\
%& $  0.586,   0.749,    0.881,   0.968,   1) $ & $ < 1.999 $ \\
%\hline
%\end{tabular}
%\end{center}
%\end{Lemma}
\begin{Proof}
For any polynomial $ \poly\in \cP_{d} $, the ratio
$r(\barn_d, \poly) $ is invariant to
multiplying both the numerator and
denominator by a constant. Thus, WLOG consider
polynomials whose leading coefficient is 1. 
Then for any $ \barn_d\in \cN_d $, $ \cP_{\barn_d} 
= (\poly_{\barn_d,1}\upto \poly_{\barn_d,d+1})$, 
is a set consisting of $ d+1 $ unique polynomials, where
each $ \poly_{\barn_d,i}, \ i\in \{1\upto d+1\} $ 
is that polynomial with 0 area in all intervals 
in $ \barI_{\barn_d} $ except $ I_{\barn_d,i}$.

\textbf{Case $ \mathbf{d = 0} $:} 
Here $ \cN_0=\{(0,1)\} $ and is a singleton set. 
Since any $ h\in\cP_0$ is a constant
value, $ \int_0^{1} |h| = |\int_0^{1} h |$. Therefore
$ r_0^{\star}=\max_{\poly \in \cP_0}
r(\barn_{d},h) = 1$.

\textbf{Case $ \mathbf{d = 1} $:} Let $ \barn_1=(0,m,1) $.
In this case $ \poly_{\barn_d,1}(x) = x-m/2  $
and $ \poly_{\barn_d,2}(x) = x-(1+m)/2  $.
Using Lemma~\ref{lem:zeroish}, 
\begin{align*}
r_1(\barn_d) 
&= \max_{\poly \in \cP_{\barn_d}}r(\barn_d,h)
= \max\{r(\barn_d, \poly_{\barn_d,1}),
r(\barn_d,\poly_{\barn_d,2})\}\\
&= \max\Big\{ \frac{m^2/4+(1-m/2)^{2}}{1-m},
\frac{(1-m)^2/4+((1+m)/2)^{2}}{m}\Big\}.
\end{align*}
$ r_1(\barn_d)  $ is minimized for $ m^{\star} = 1/2 $,
giving $ r^{\star}_1=(1/16+9/16)/(1/2)=1.25 $.

\textbf{Case $ \mathbf{d = 2} $:}
By symmetry, the minimizing node partition
is symmetric about $ 0.5 $. Thus WLOG let $ \barn_2 =(0,m,1-m,1) $ for 
some $ m\le 0.5 $.  Among the $ d+1=3 $ polynomials 
in $ \cP_{\barn_2} $, by symmetry of $ \barn_2 $, 
$ r_{2}(\poly_{\barn_d,1})  =r_{2}(\poly_{\barn_d,3})$. 
Thus we consider the larger ratio across only two polynomials,
$ \poly_{\barn_d,2}, \poly_{\barn_d,3} $.

Denote the polynomial as $ \poly_{\barn_d,2}(x) =
(x-a_{2})^2-b_{2}^2 $ and upon setting the respective integrals to $ 0 $,
\[\Big|\frac{m^3}{3}-a_{2}m^2+(a_{2}^2-b_{2}^2)m\Big|
=0, \ \Big|\frac{1-(1-m)^3}{3}-a_{2}(1-(1-m)^2)
+(a_{2}^2-b_{2}^2)m\Big|=0
\]
\[\implies a_{2}=\frac12, b_{2}^{2}=\frac{3(m^2-m)+1}{9}.\]
Representing $ \poly_{\barn_d,3}(x) = (x-a_{3})^2-b_{3}^2 $
and repeating the same steps,
\[
\Big|\frac{m^3}{3}-a_{3}m^2+(a_{3}^2-b_{3}^2)m\Big|
=0,\ \Big|\frac{(1-m)^3-m^3}{3}-a_{3}((1-m)^2-m^2)
+(a_{3}^2-b_{3}^2)(1-2m)\Big|=0
\]
\[\implies a_{3}=\frac13, b_{3}^{2}=\frac{4m^2-6m+3}{3}.\]

The corresponding $ r(\barn_d,\poly_{\barn_d,2}) $ and 
$ r(\barn_d,\poly_{\barn_d,3}) $ are given by
\[\frac{8\left(\frac{1-3m(1-m)}{9}\right)^{3/2}}{m(1-m)}+1,
\,
\frac{2\left(\frac{(2m-1)(2m-2)+1}{3}\right)^{3/2}}{(2m-1)(m-1)}-1. \]

From simultaneously minimizing the above expressions by equating 
them, the optimal $  m $ is the root of 
\begin{align*}
q_{2}(m)&=-\frac{26624}{729} m^{14}+\frac{193280}{729}m^{13}
- \frac{211024} {243} m^{12} + \frac{3703648}{2187} m^{11} 
- \frac{4790776}{2187} m^{10}+ \frac{39108232}{19683} m^9 \\
&\phantom{=}- \frac{8554775}{6561} m^8+ \frac{12357280}{19683} m^7 
- \frac{13004032}{59049} m^6 + \frac{1061792}{19683} m^5 
- \frac{4350752}{531441} m^4 + \frac{246976}{531441}m^3 \\
&\phantom{=}+ \frac{11840}{177147} m^2 - \frac{6656}{531441}m 
+ \frac{256}{531441}
\end{align*}
near $ 0.26 $. Thus the optimal $m^{\star}\approx 0.2599$
and the corresponding $r_2^{\star}\approx 1.423$.

\textbf{Case $ \mathbf{d = 3} $:}
By symmetry, as before, WLOG let $ \barn_d=(0,m,0.5,1-m,1) $.
This reduces the search space to just two polynomials, 
$ \poly_{\barn_d,1} $, $\poly_{\barn_d,2}  $. 
The optimal $ m$ occurs as the root of
\input{poly69.tex} 
near $ 0.155 $. This gives $ m^{\star}\approx 0.1548 $
and the corresponding $ r^{\star}_{3}\approx 1.559 $.

For degrees $ 4\le d\le 8 $, we use numerical
methods on top of Lemma~\ref{lem:zeroish} to derive 
$ \barn_d\in \cN_d $ and the corresponding $ r_d(\barn_d) $.
These values populate the second table in Lemma~\ref{lem:optnodes}.
\end{Proof}


==> appenstitch.tex <==
\section{The Compare and Stitch Routines}
\subsection{Proof of Lemma~\ref{lem:binarycomp}}
%\begin{Lemma}
%\label{lem:binarycomp}
%For any empirical distribution
%$ \barhatp \in \Delta_{\mathrm{emp,n}}$, 
%there exists $  \barhatp' \in \Delta_{\mathrm{bin,n}}$ 
%such that
%\[
%\lone{\starf_{\barI_{\barhatp'}}-f} \le
%\lone{\starf_{\barI_{\barhatp}}-f}, \
%\sum_{\hatp \in \barhatp'}
%\epsilon\sqrt{\hatp}
%\le
%\sum_{\hatp\in \barhatp}
%\frac{1}{\sqrt{2}-1}\epsilon\sqrt{\hatp},
%\]
%where $ \starf_{\barI} $ is the polynomial closest to 
%$ f $ across in interval $ \barI $.
%\end{Lemma}
\begin{Proof}
As observed in Equation~\eqref{eqn:empiricaldist},
any $ \hatp\in \barhatp\in \Delta_{\textrm{emp,n}} $
is an integral multiple of $ 1/n $. Observing that $ \log _{2}n $ 
is an integer, we may decompose $ \hatp $ along its 
binary expansion as \[ \hatp = \sum_{j=0}^{\log_{2} n} 2^{-j}b_{j},\]
for some $ b_{j}\in\{0,1\} $, $ j\in \{1\upto \log_{2}n\} $. 
Replace each $ \hatp \in \barhatp$ with the vector 
$ (2^{-0}b_{0}, 2^{-1}b_{1},\cdots) $ to obtain 
$\barhatp'\in \Delta_{\mathrm{bin,n}}$.
From the property of the geometric sum,
\[\sum_{j=0}^{\log_{2}n} \sqrt{2^{-j}b_{j}}
\overset{}{\le}
\frac{\sqrt{\hatp}}{\sqrt2-1}.\]
Finally $\lone{\starf_{\barI_{\barhatp'}}-f} 
\le
\lone{\starf_{\barI_{\barhatp}}-f}$
since $\barI_{\barhatp'}$ being a finer partition
than $ \barI_{\barhatp} $, 
$ \starf_{\barI_{\barhatp'}} $ is a closer approximation to $ f $ 
than $ \starf_{\barI_{\barhatp}} $.
\end{Proof}

\subsection{Proof of Lemma~\ref{lem:master}}
%\begin{Lemma}
%\label{lem:master}
%Given samples $ X^{n-1}\sim f $, for some $ n $ that 
%is a power of $ 2 $, degree $ d\le 8 $ and
%the threshold $ \alpha > 2$, $ \SURF$ 
%outputs $ \hatf_{\text{SURF}} $ in time 
%$ \cO((d^\tau+\log n)n\log n) $ such that under event 
%$ \cQ_{\epsilon} $,
%\begin{align*}
%&\lone{\hatf_{\text{SURF}}-f}\\
%&\le
%\min_{\barp \in \Delta_{\mathrm{bin,n}}}
%\sum_{p \in \barp} \left(
%\frac{(r_d+1)\cdot \alpha}{\alpha-2}\cdot 
%\inf_{\poly \in \cP_d}\loneint{\barI_{\barp}}{\poly-f}\right.\\
%&\phantom{\le\min_{\barI\in 
%\Delta_{\barI}}\sum_{p \in \barp}\Big ( }
%\left.\ +\frac{r_d\cdot (\alpha\sqrt2+\sqrt{2}-1)}{\sqrt{2}-1}
%\epsilon \sqrt{(d+1)p}\right),
%\end{align*}
%where $ r_d $ is the constant corresponding
%to the $ \EQ $ routine given in Theorem~\ref{thm:polyblack}.
%\end{Lemma}
%The above lemma, along with Lemma~\ref{lem:binarycomp} 
%that establishes the approximating power 
%of these binary partitions allow us to show 
%Theorem~\ref{thm:interhistopt}.
\begin{Proof}
For any interval $ I $, let 
\[ f^{\star}_{I} \ed \arg \min_{h\in \cP_{d}}\loneint{I}{h-f},\]
and for any partition $ \barI $, let $  f^{\star}_{\barI}  $
be the piecewise polynomial that equals 
$ f^{\star}_{I} $ in each $ I\in \barI $.
For simplicity let 
$ I_{\barhatp}\ed I_{\barhatp_D} $ denote the final
partition and $ \barhatp \ed \barhatp_{D} $ the 
corresponding empirical distribution. Consider any 
$ \barhatpp \in \Delta_{\mathrm{bin,n}}$ 
and its associated interval partition, 
$ \barI_{\barhatpp} $.
Two interval partitions $ \bar{I}_1,\bar{I}_2 $ 
corresponding to binary distributions 
have the following property:
Any interval in $ \bar{I}_1 $ is either 
completely contained within some interval in $ \bar{I}_2 $, 
or is a union of contiguous intervals from $ \bar{I}_2 $.
As a result $ \barI_{\barhatp} $ may partitioned 
into three classes of intervals:
%
\begin{figure}[H]
\centering
\includegraphics[scale=0.85]{bin1.pdf}
\caption{Illustration of $ \barI_{\barhatp} $ being partitioned into 
$ \barI_{\barhatp}^{1} $, $  \barI_{\barhatp}^{2} $ and $  \barI_{\barhatp}^{3} $ using $ \barI_{\barp} $.}
\label{fig:bin1}
\end{figure}
%
\begin{itemize}
\item $ \barI^1_{\barhatp} $, composed of intervals 
that are equal to some interval in $ \barI_{\barp} $,
\item $ \barI^2_{\barhatp} $, that consists of intervals 
that lie strictly within some interval in $ \barI_{\barhatpp} $,
\item $ \barI^3_{\barhatp} $, containing intervals
that are unions of more than one interval from $ \barI_{\barp} $.
\end{itemize}
This is shown in Figure~\ref{fig:bin1}.
Lemmas~\ref{lem:start},~\ref{lem:middle},~\ref{lem:end} 
address each of these intervals separately. Combining the
lemmas, 
\begin{align*}
\lone{\hatf_{\barI_{\barhatp}}-f}
&=\loneint{\barI^1_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f}
+\loneint{\barI^2_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f} 
+\loneint{\barI^3_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f} \\
&\overset{}{\le} (r_d+1)\cdot\loneint{\barI^1_{\barhatp}}
{\starf_{\barI_{\barp}}-f}
+ \sum_{I \in \barI^{1}_{\barp}}
r_d\cdot \epsilon \sqrt{(d+1)p_I}\\
&\phantom{\le} +\frac{(r_d+1)\cdot \alpha}{\alpha-2}\cdot 
\loneint{\barI^2_{\barhatp}}
{\starf_{\barI_{\barp}}-f}+\frac{1}{\alpha-1}
%for camera ready -2
\sum_{ I\in \barI^2_{\barp} }
r_d\cdot \epsilon \sqrt{(d+1)p_I}\\
&\phantom{\le} +(r_d+1)\cdot 
\loneint{\barI^{3}_{\barhatp}}{\starf_{\barI_{\barp}}-f}
+\frac{\alpha\sqrt2+\sqrt{2}-1}{\sqrt{2}-1} \sum_{I\in \barI^{3}_{\barp}}
r_d\cdot \epsilon \sqrt{(d+1)p_I}\\
&\overset{(a)}{\le} \frac{(r_d+1)\cdot \alpha}{\alpha-2}
\lone{\starf_{\barI_{\barp}}-f}
+\frac{\alpha\sqrt2+\sqrt{2}-1}{\sqrt{2}-1}
\sum_{I\in \barI_{\barp}} 
r_d\cdot \epsilon \sqrt{(d+1)p_I},
\end{align*}
where $ (a) $ follows since $ \alpha>2 \Rightarrow
1/(\alpha-1)<1<(\alpha\sqrt2+\sqrt{2}-1)/(\sqrt{2}-1)$.
\end{Proof}

\begin{Lemma}
\label{lem:start}
For the final partition $ \barI_{\barhatp} $ in the run of $ \STITCH $
and any $ \barp\in \Delta_{\mathrm{bin,n}} $, let 
$\barI^{1}_{\barhatp}\subseteq \barI_{\barhatp} $ 
be the intervals that intersect with $ \barI_{\barp} $.
Let $\barI^{1}_{\barp}=\barI^{1}_{\barhatp}\subseteq \barI_{\barp} $ 
denote the corresponding collection in $ \barI_{\barp}$. Then,
\[\loneint{\barI^1_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f}
\le (r_d+1)\cdot\loneint{\barI^1_{\barhatp}}
{\starf_{\barI_{\barp}}-f}
+ \sum_{I \in \barI^{1}_{\barp}}
r_d\cdot \epsilon \sqrt{(d+1)p_I},
\]
\end{Lemma}
\begin{Proof}
Follows from Theorem~\ref{thm:polyblack}
and noticing that intervals in $ \barI^{1}_{\barhatp} $ 
and $ \barI^{1}_{\barhatpp} $ coincide.
\end{Proof}

\begin{Lemma}
\label{lem:middle}
For the final partition $ \barI_{\barhatp} $ 
in the run of $ \STITCH $ and any 
$ \barp\in \Delta_{\mathrm{bin,n}} $, let 
$\barI^{2}_{\barhatp}\subseteq \barI_{\barhatp} $ 
be the intervals that do not intersect with, and strictly lie in 
some interval in $ \barI_{\barp} $.
Let $\barI^{2}_{\barp}\subseteq \barI_{\barp} $ 
be the corresponding intervals that 
contain $ \barI^{2}_{\barhatp}$. Then,
\begin{align*}
\loneint{\barI^2_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f}
&\overset{}{\le} \frac{(r_d+1)\cdot \alpha}{\alpha-2}\cdot
\loneint{\barI^2_{\barhatp}}
%for camera -2
{\starf_{\barI_{\barp}}-f}+\frac{1}{\alpha-1}
\sum_{ I\in \barI^2_{\barp} }
r_d\cdot \epsilon \sqrt{(d+1)p_I}.
\end{align*}
\end{Lemma}
\begin{Proof}
Notice that all intervals in $ \barI^2_{\barhatp} $ are strictly 
contained within some interval in $ \barI^{2}_{\barp} $. 
Using this, we further partition 
$ \barI^2_{\barhatp} $ using intervals in $ \barI^2_{\barp} $. 
Fix an $ I\in \barI^{2}_{\barp} $ and let
$ \barI \in \barI^2_{\barhatp} $ be intervals
whose union gives $ I$. 
Let $ \barhatp_{\barI}\subseteq\barhatp $ denote the 
empirical probabilities corresponding to $ \barI $
and let $ p_I $ denote the empirical probability 
under $ I $.
%
\begin{figure}[H]
\centering
\includegraphics[scale=0.85]{bin2.pdf}
\caption{Illustration of $ \barI\in \barI^{2}_{\barhatp}$, $ \barI_{\barhats_{I}} $ and
$ \barI_{\barhats_{I}^{1}} $ corresponding to a
particular $ I\in \barI^{2}_{\barp}$.}
\label{fig:bin2}
\end{figure}
%
While $ \barhatp_{\barI} $ is a sub-distribution
in general, WLOG assume $ \barhatp_{\barI} $ is 
a distribution.
Now, at some point in the run of $\STITCH$,
$ \MERGE $ was called with $ \hatf_{I,\EQ} $,
$ \barI $, 
$ \barhatp_{\barI}  $, and it was in-turn declared 
that $ \barI $ was not to be merged into $ I $. 
Therefore, for the 
$ \lemerge_{\barI,\gamma }(\hatf_{I,\EQ}) $
attaining binary distribution,
$ \barhats_{I} \in \Delta_{\mathrm{bin,n}, \ge \barhatp_{\barI}  }$,
$ \del_{I_{\barhats_{I}}}(\hatf_{I,\EQ}) - \thr_{\barhats_{I},\gamma}\ge 0$.
It follows that 
\begin{align*}
\sum_{\hats \in \barhats_{I}}
\alpha \cdot r_d\cdot \epsilon \sqrt{(d+1)\hats}
&=\thr_{\barhats_{I},\gamma}\le \del_{I_{\barhats_{I}}}(\hatf_{I,\EQ}) \\
&=\loneint{I}
{\hatf_{I,\EQ}-\hatf_{\barI_{\barhats_{I}}}}\\
&\le \loneint{I}{\hatf_{I,\EQ}-f}
+\loneint{I}{f-\hatf_{\barI_{\barhats_{I}}}}\\
&\overset{(a)}{\le}
(r_d+1)\cdot \loneint{I}{\starf_{I}-f}
+r_d\cdot \epsilon \sqrt{(d+1)p_I}\\
&\phantom{\le}+(r_d+1)\cdot
\loneint{I} {\starf_{\barI_{\barhats_{I}}}-f}
+\sum_{\hats \in {\barhats_{I}}} 
r_d\cdot \epsilon \sqrt{(d+1)\hats}\\
&\overset{(b)}{\le} 2(r_d+1)\cdot \loneint{I}{\starf_{I}-f}
+r_d\cdot \epsilon \sqrt{(d+1)p_I}+\sum_{\hats \in {\barhats_{I}}} 
r_d\cdot \epsilon \sqrt{(d+1)\hats},
\end{align*}
where $ (a) $ follows from in Theorem~\ref{thm:polyblack}, 
$ (b) $ follows since $ I $ being the union of 
$ \barI_{\barhatp_{I}} $ is also the union of 
$ \barI_{\barhats_{I}} $,
and $\starf_{I} $ is therefore a coarser approximation 
to $ f $ than $ \starf_{\barI_{\barhats_{I}}} $, 
giving rise to a larger $ \ell_{1} $ distance.
Rearrange this to obtain
\begin{equation}
\label{eqn:middleone}
\sum_{\hats \in \barhats_{I}}
r_d\cdot \epsilon \sqrt{(d+1)\hats}
\le 
\frac{1}{{\alpha-1} }\cdot\left(
2(r_d+1)\cdot \loneint{I}{\starf_{I}-f}
+r_d\cdot \epsilon \sqrt{(d+1)p_I}\right).
\end{equation}
%
Consider a fixed $ I' \in \barI_{\barhats_{I}}$ and let 
$ \barI' \in \barI$ be the intervals 
under $ \barI $ whose union gives $ I' $.
%Suppose if $ \barI' = I'$ is a singleton, we stop,
%noting that for this interval, $ \hats_{I'} =\hatp_{I'} $.
%This occurs for the two rightmost intervals of $ \barI_{\barhats_{I}} $
%in Figure~\ref{fig:bin2}.
%
%Otherwise, 
We recursively use the same argument to 
bound the LHS of Equation~\eqref{eqn:middleone}.
This is shown for the leftmost interval of $ \barI_{\barhats_{I}} $
in Figure~\ref{fig:bin2}.
Let $ \barhatp_{\barI'} $ be the corresponding 
probabilities under $ \barI'  $ and let $ \hats_{I'} $
denote the empirical probability under $ I' $.
Notice that in some previous step of $ \STITCH $, 
as was for $ I $, $ \MERGE $ was invoked with 
$ \hatf_{I',\EQ} $, $ \barI' $, $ \barhatp_{\barI'} $, 
for which 
$ \lemerge_{\barI',\gamma}(\hatf_{I',\EQ})\ge 0 $. 
Repeat the same procedure as above to obtain
\begin{align}
\nonumber
\sum_{\hats \in \barhats_{I'}}
r_d\cdot \epsilon \sqrt{(d+1)\hats}
&\le
\frac{1}{{\alpha-1} }\cdot\left(
2(r_d+1)\cdot \loneint{I'}{\starf_{I'}-f}
+r_d\cdot \epsilon \sqrt{(d+1)\hats_{I'}}\right)\\
\label{eqn:middleoneandhalf}
&\overset{(a)}{\le} \frac{1}{{\alpha-1} }\cdot\left(
2(r_d+1)\cdot \loneint{I'}{\starf_{I}-f}
+r_d\cdot \epsilon \sqrt{(d+1)\hats_{I'}}\right),
\end{align}
where $ \barhats_{I'} $ here is the binary distribution
which attains 
$ \lemerge_{\barI',\gamma}(\hatf_{I',\EQ}) $,
and $ (a) $ 
follows because $ I' $ being an interval within $ I $,
$ \starf_I $ is a coarser approximation to $ f $
than $ \starf_{I'} $. 
Summing Equation~\eqref{eqn:middleoneandhalf} 
for each such $ I' $, accumulate the distribution 
$ \barhats^{1}_{I} \ed (\cup_{I'\in \barI_{\barhats_{I}}}\barhats_{I'}) $,
and using Equation~\eqref{eqn:middleone}, the inequality,
\begin{equation}
\label{eqn:middletwo}
\sum_{\hats\in \barhats^{1}_{I}}
r_d\cdot \epsilon \sqrt{(d+1)\hats} 
\le \left(\frac{1}{\alpha-1} + \frac{1}{(\alpha-1)^2}\right)\cdot
2(r_d+1)\cdot \loneint{I}{\starf_{I}-f}
+\frac{1}{\alpha-1} \cdot r_d\cdot \epsilon \sqrt{(d+1)p_I}.
\end{equation}
Notice that while both 
$ \barhats_{I},\barhats^{1}_{I}\in \Delta_{\mathrm{bin,n},\ge \barhatp_I} $,
$\barhats^{1}_{I}$ is at least one notch closer to $ \barhatp_{I} $ as
$ \barhats^{1}_{I}\in \Delta_{\mathrm{bin,n}, < \barhats_{I}} $.
Since the number of binary distributions is finite,
on recursively using this argument,
summation across $ \barhatp_{I} $ is eventually
obtained on the LHS. Iterating on this procedure yields 
the upper bound
\begin{align*}
\sum_{\hatp \in \barhatp_{\barI}}
r_d\cdot \epsilon \sqrt{(d+1)\hatp}
&\le \left(\frac{1}{\alpha-1} + \frac{1}{(\alpha-1)^2}+\cdots\right)\cdot
2(r_d+1)\cdot \loneint{I}{\starf_{I}-f}
+\frac{1}{\alpha-1} r_d\cdot \epsilon \sqrt{(d+1)p_I}\\
&\overset{(a)}{\le} \frac{2(r_d+1)}{\alpha-2}\cdot
\loneint{I}{\starf_{I}-f}+\frac{1}{\alpha-1}\cdot
r_d\cdot \epsilon \sqrt{(d+1)p_I},
\end{align*}
where $ (a) $ follows since $ \alpha>2 $.
Repeating this argument across each 
$I \in \barI^2_{\barp} $,
\begin{equation}
\label{eqn:middlethree}
\sum_{I\in \barI^2_{\barhatp}}
r_d\cdot \epsilon \sqrt{(d+1)\hatp_I}
\le \frac{2(r_d+1)}{\alpha-2}\cdot
\loneint{\barI^2_{\barhatp}}
{\starf_{\barI_{\barp}}-f}+\frac{1}{\alpha-1}
\sum_{ I\in \barI^2_{\barp} }
r_d\cdot \epsilon \sqrt{(d+1)p_I}.
\end{equation}
This finally gives us
\begin{align*}
\loneint{\barI^2_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f}
&\overset{(a)}{\le} (r_d+1)\cdot
\loneint{\barI^2_{\barhatp}}{\starf_{\barI_{\barhatp}}-f}
+\sum_{I \in \barI^{2}_{\barhatp}}
r_d\cdot \epsilon \sqrt{(d+1)\hatp_I}\\
&\overset{(b)}{\le} (r_d+1)\cdot
\loneint{\barI^2_{\barhatp}}{\starf_{\barI_{\barp}}-f}
+\sum_{I \in \barI^{2}_{\barhatp}}
r_d\cdot \epsilon \sqrt{(d+1)\hatp_I}\\
&\overset{}{\le} (r_d+1) \left(1+\frac{2}{\alpha-2}\right)
\loneint{\barI^2_{\barhatp}}
{\starf_{\barI_{\barp}}-f}+\frac{1}{\alpha-1}
\sum_{ I\in \barI^2_{\barp} }
r_d\cdot \epsilon \sqrt{(d+1)p_I},
\end{align*}
where $ (a) $ follows from Theorem~\ref{thm:polyblack}, 
$ (b) $ follows since, by definition, intervals in 
$ \barI^{2}_{\barhatp} $ lie within those in 
$ \barI^{2}_{\barp} $, and thus $ \starf_{\barI_{\barp}} $
is a coarser approximation to $ f $ than $ \starf_{\barI_{\barhatp}} $
in $ \barI_{\barhatp}^{2} $,
and finally $ (c) $ follows by plugging in Equation~\eqref{eqn:middlethree}.
\end{Proof}

\begin{Lemma}
\label{lem:end}
For the final partition $ \barI_{\barhatp} $ in the run of $ \STITCH $
and any $ \barp\in \Delta_{\mathrm{bin,n}} $, let 
$\barI^{3}_{\barhatp}\subseteq \barI_{\barhatp} $ 
be intervals that are unions of more 
than one interval from $ \barI_{\barp} $.
Let $\barI^{3}_{\barp}\subseteq \barI_{\barp} $
be the corresponding intervals whose union gives 
$ \barI^{3}_{\barhatp}$. Then,
\begin{align*}
\loneint{\barI^{3}_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f}
\le (r_d+1)\cdot \loneint{\barI^{3}_{\barhatp}}{\starf_{\barI_{\barp}}-f}
+\frac{\alpha\sqrt2+\sqrt{2}-1}{\sqrt{2}-1} \sum_{I\in \barI^{3}_{\barp}}
r_d\cdot \epsilon \sqrt{(d+1)p_I}.
\end{align*}
\end{Lemma}
\begin{Proof}
Fix an $ I \in \barI^{1}_{\barhatp}$
and let $ \hatp_{I} $ be its empirical probability. 
Let $ \barI_{\barp, I} \in \barI_{\barp} $ 
indicate intervals
under $ \barI_{\barp} $ whose union gives 
$ I $ and let $ \barp_{I} \subseteq \barp$ denote
the corresponding empirical probabilities under
$ \barI_{\barp,I}$.
In run of $ \STITCH $, let the interval 
collection that was merged to create $ I $ be denoted 
by $ \barI_{\barhatp,I} $, and its collection of empirical probabilities 
by $ \barhatp_{I}$. While $ \barp_{I} $ is a 
sub-distribution in general, WLOG assume
it is a distribution. This also implies 
$ \barhatp_{I}$ is a distribution.
%using which we may
%denote $ \barI_{\barp'}=\barI $, $ \barI_{\barhatp'} = \bar{K}$.

Using $ \barI_{\barhatp,I}$, separate $ \barI_{\barp,I} $ into
\begin{itemize}
\item $ \barI_{\barp,I}^{1} $, consisting of intervals
in $ \barI_{\barp,I}$ that are equal to, or unions of 
intervals from $ \barI_{\barhatp,I} $.
\item $ \barI_{\barp,I}^{2} $, intervals in $ \barI_{\barp,I}$
that lie strictly inside some interval in $ \barI_{\barhatp,I} $.
\end{itemize}

Let $ \barI_{\barhatp,I}^2\subseteq $ 
be the corresponding intervals in 
$ \barI_{\barhatp,I} $ 
that contain $ \barI_{\barp,I}^{2} $.
Let $ \barp^{1}_{I} $, $ \barp^{2}_I $ be empirical probabilities
corresponding to $ \barI_{\barp,I}^{1} $, $ \barI_{\barp,I}^{2} $
respectively. 
Similarly let $ \barhatp^{2}_I $ correspond to $ \barI_{\barhatp,I}^{2} $.
This is shown in Figure~\ref{fig:bin3}, where the arrow indicates
the collection of intervals merged by $ \STITCH $.
%
\begin{figure}[H]
\centering
\includegraphics[scale=0.85]{bin3.pdf}
\caption{Illustration of proof construction for a particular $ I\in \barI^{3}_{\barhatp}$.}
\label{fig:bin3}
\end{figure}
%
Modify $ \barI_{\barp,I} $ to obtain 
a new partition 
$ \barJ_{\barp,I} \ed \barI_{\barp,I}^{1} \cup \barI_{\barhatp,I}^2$.
Now each interval in $ \barJ_{\barp,I} $ is equal to, 
or is a union of intervals from $ \barI_{\barhatp,I} $. 
Equivalently, if $ \barhats $ is the 
empirical distribution corresponding to 
$ \barJ_{\barp,I} $, 
$ \barhats \in \Delta_{\mathrm{bin,n},\ge \barhatp_{I}} $.
Since $ I $ was merged when the merging routine
was called with $ \hatf_{I,\EQ} $,
$ \barI_{\barhatp,I}$, $ \barhatp_{I}$,
it implies
$ \thr_{\barhats,\gamma} \ge \del_{I_{\barhats}}(\hatf_{I,\EQ}) $. 
Therefore
\begin{align}
\nonumber
\loneint{I}{\hatf_{\barI_{\barhatp}}-f}&\le \loneint{I}{\hatf_{\barJ_{\barp,I}}-f} 
+ \loneint{I}{\hatf_{\barI_{\barhatp}}-\hatf_{\barJ_{\barp,I}}} \\
\nonumber
&\overset{(a)}{=} \loneint{I}{\hatf_{\barJ_{\barp,I}}-f}  + \del_{I_{\barhats}}(\hatf_{I,\EQ}) \\
\nonumber
&\le \loneint{I}{\hatf_{\barJ_{\barp,I}}-f}  + \thr_{{\barhats},\gamma}\\
\nonumber
&\overset{(b)}{=} \loneint{\barJ_{\barp,I}}{\hatf_{\barJ_{\barp,I}}-f}  
+\thr_{{\barhats},\gamma}\\
\nonumber
&= \loneint{\barJ_{\barp,I}}{\hatf_{\barJ_{\barp,I}}-f}  + \alpha
\sum_{s\in\barhats}
r_d\cdot \epsilon \sqrt{(d+1)s}\\
\nonumber
&\overset{(c)}{=} \loneint{\barI^1_{\barp,I}}{\hatf_{\barI^{1}_{\barp,I}}-f} 
+ \alpha\sum_{p\in\barp^{1}_{I}}
r_d\cdot \epsilon \sqrt{(d+1)p}\\
\nonumber
&\phantom{=}
+ \loneint{\barI^2_{\barhatp,I}}{\hatf_{\barI^{2}_{\barhatp,I}}-f}
+ \alpha\sum_{\hatp\in\barhatp^{2}_{I}}
r_d\cdot \epsilon \sqrt{(d+1)\hatp}\\
\nonumber
&\overset{(d)}{=} \loneint{\barI^1_{\barp,I}}{\hatf_{\barI_{\barp}}-f}  
+ \alpha\sum_{p\in\barp^{1}_{I}}
r_d\cdot \epsilon \sqrt{(d+1)p}\\
\label{eqn:threeone}
&\phantom{=}
+ \loneint{\barI^2_{\barhatp,I}}{\hatf_{\barI^{2}_{\barhatp,I}}-f}
+ \alpha\sum_{\hatp\in\barhatp^{2}_{I}}
r_d\cdot\epsilon \sqrt{(d+1)\hatp},
\end{align}
where $ (a) $ follows since by definition,
$\hatf_{\barI_{\barhatp}} = \hatf_{I,\EQ} $
in interval $ I $,
$ (b) $ follows since $ \barJ_{\barp,I} $ being 
a partition of $ I $ lies in the same region as $ I $, 
$ (c) $ follows since
$ \barJ_{\barp,I} = \barI_{\barp,I}^{1} \cup \barI_{\barhatp,I}^2$,
and $ (d) $ follows since 
$ \hatf_{\barI_{\barp}} = \hatf_{\barI^{1}_{\barp,I}}$
in $ \barI_{\barp,I}^{1} $ as $ \barI^{1}_{\barp,I}\subseteq \barI_{\barp}$. 

Now consider an interval $ I' \in \barI_{\barhatp,I}^{2} $. 
Since $\barI_{\barhatp,I}^{2}\subseteq \barI_{\barhatp,I}$, 
and since $ \barI_{\barhatp,I} $, by definition, are
intervals that were merged to produce $ I $,
it follows that $ I' $ in turn was an interval that was merged into in
some previous step of $ \STITCH $. 
As before, let the intervals that were merged
to generate $ I' $ be denoted by $ \barI_{\barhatp,I'} $.
Further, by definition of
$ \barI_{\barhatp,I}^{2}$, all intervals in it
occur as unions of those in $ \barI^{2}_{\barp,I}$, 
and so does $ I' $.
Let $ \barI_{\barp,I'} \subseteq \barI^{2}_{\barp,I} $ be 
these intervals whose union gives $ I' $.
Repeat the same argument as above to obtain
\begin{align}
\nonumber
\loneint{I'}{\hatf_{\barI^{2}_{\barhatp}}-f}
&\le  \loneint{\barI^1_{\barp,I'}}{\hatf_{\barI_{\barp}}-f}  
+ \alpha\sum_{p\in\barp^{1}_{I'}}
r_d\cdot \epsilon \sqrt{(d+1)p}\\
\label{eqn:threetwo}
&\phantom{\le}
+ \loneint{\barI^2_{\barhatp,I'}}{\hatf_{\barI^{2}_{\barhatp,I'}}-f}
+ \alpha\sum_{\hatp\in\barhatp^{2}_{I'}}
r_d\cdot \epsilon \sqrt{(d+1)\hatp},
\end{align}
where each of  $ \barI^{1}_{\barp,I'} $, $ \barp^{1}_{I'} $, 
$ \barI^2_{\barhatp,I'} $ and $ \barhatp^{2}_{I'}$ are 
defined in exactly the same manner as was for $ I $,
but by replacing $ I' $ in all definitions.
Since $ \barI^{1}_{\barp,I'} 
\subseteq \barI^{2}_{\barp,I}\subseteq \barI_{\barp}$,
substituting Equation~\eqref{eqn:threetwo}
into~\eqref{eqn:threeone},
a larger portion of $ I $ is bounded using the 
difference $ \loneint{}{\hatf_{\barI_{\barp}} -f}$.
Upon repeating the same argument for all
$ \loneint{}{\hatf_{\barI_{\barhatp}}-f}$ terms that 
remain, a bound on the RHS is obtained that 
consists exclusively of $ \loneint{}{\hatf_{\barI_{\barp}}-f} $.
The entire procedure is shown in Figure~\ref{fig:bin3}.

Further, from Lemma~\ref{lem:treegeosum}, 
the sum of all the $ \epsilon $-deviation terms 
that results on the RHS from repeating the 
argument is bounded by $ \sqrt2/(\sqrt{2}-1) $ times
the total $ \epsilon $-deviation in $ \barI_{\barp}^{3} $. This results in
\begin{align*}
\loneint{I}{\hatf_I-f} &\le \loneint{I}{\hatf_{\barI_{\barp}}-f}
+ \frac{\alpha}{\sqrt{2}-1} \sum_{p\in\barp_{I}}
r_d\cdot \epsilon \sqrt{(d+1)p}\\
&\overset{(a)}{\le} (r_d+1)\cdot \loneint{I}{\starf_{\barI_{\barp}}-f}
+ \left(1+\frac{\alpha\sqrt2}{\sqrt{2}-1}\right) \sum_{p\in\barp_{I}}
r_d\cdot\epsilon \sqrt{(d+1)p},
\end{align*}
where $ (a) $ follows from Theorem~\ref{thm:polyblack}.
Repeating across $I\in \barI^{3}_{\barhatp}  $ gives 
\begin{align*}
\loneint{\barI^{3}_{\barhatp}}{\hatf_{\barI_{\barhatp}}-f}
\le (r_d+1)\cdot \loneint{\barI^{3}_{\barhatp}}{\starf_{\barI_{\barp}}-f}
+ \left(1+\frac{\alpha\sqrt2}{\sqrt{2}-1}\right) \sum_{I\in \barI^{3}_{\barp}}
r_d\cdot \epsilon \sqrt{(d+1)p_I}.
\end{align*}
\end{Proof}

\begin{Lemma}
\label{lem:treegeosum}
Suppose in the run of $ \STITCH $, a collection of consecutive 
intervals $ \barI_1 $ was merged in $ k-1 $ steps 
to generate $ \barI_k $, and suppose 
$ \barI_2\upto \barI_{k-1} $ are 
the intermediate interval collections. Then, 
\[\sum_{i=1}^k
\sum_{I\in \barI_i}\sqrt{\hatp_I}
\le \sum_{I\in \barI_1} \frac{\sqrt2}{\sqrt{2}-1}\sqrt{\hatp_I}.
\]
\end{Lemma}
\begin{Proof}
WLOG assume $ \barhatp_{\barI_{1}} $ is a distribution, 
which also implies $ \barhatp_{\barI_{i}} $ is a distribution 
$ \forall i\in \{2\upto k\} $. Notice that
for any $ i\in \{2\upto k\} $,
$ \barhatp_{\barI_{i}}\in \Delta_{\mathrm{\mathrm{bin,n}},
\ge \barhatp_{\barI_{i-1}}} $.
Thus $ |\barI_{i}| \le 1/2\cdot  |\barI_{i-1}|$, 
where $ |\barI| $ denotes the number of intervals in $ \barI $.
By concavity of $ \sqrt{x} $ for $ x\ge 0 $, the sum 
$ \sum_{I\in \barI_{i}}\sqrt{\hatp_I} $ is maximized
for a given $ \barhatp_{\barI_{i-1}} $, 
if $  |\barI_{i-1}| = 2 \cdot |\barI_{i}|$.
Since this equality is attained iff $ \barhatp_{\barI_{i-1}} $ is
the uniform distribution over $ |\barI_{i-1}| $ elements
and $ \barhatp_{\barI_{i}} $ is uniform over 
$ |\barI_{i}| = 1/2\cdot |\barI_{i-1}| $ elements,
\[\sum_{I\in \barI_i}\sqrt{\hatp_I} 
\le \frac{1}{\sqrt{2}}\sum_{I\in \barI_{i-1}}\sqrt{\hatp_I}.\]
This implies 
\[\sum_{i=1}^k
\sum_{I\in \barI_i}\sqrt{\hatp_I}
\le \sum_{i=1}^k \left(\frac{1}{\sqrt{2}}\right)^{i-1}\cdot
\sum_{I\in \barI_1} \sqrt{\hatp_I}
\le \frac{\sqrt2}{\sqrt{2}-1}\sum_{I\in \barI_1} \sqrt{\hatp_I}.
\]
\end{Proof}

==> backup.tex <==
\section{The $ \SPLIT $ Routine}
\label{sec:singlep}
For an interval $ I $ and $ \eta > 0$ let 
$ \tilde{q} \in\cP_{d} $ be an estimate such that 
for constants $ c_{3}, c_{4} $, 
\begin{align*}
	\loneint{I}{\tilde{q}-f}
	\le c_{3}\OPT_{\cP_{d}} (f) +c_{4}\akkint{d+1}{I}{\hatf - f} +\eta.
\end{align*}
$ \SPLIT $ transforms $ \tilde{q} $ 
to $ \hatq $ such that it 
achieves a $ 2 $-factor approximation 
for $ \cP_{d} $.

Given an $ I\subseteq \reals $, $ \tilde{q}_{\cA_{d+1}, I} $ and numbers
$l\ge 0$, $c_1\ge 0$ such that $c_1<1/2$,
$ \SPLIT $ returns a partition $ \barJ(I, c_{1}, l) $ of $ I $ 
and a piecewise $ \hatq_{I} = \hatq_{\barJ(I, c_{1}, l )} $
that is a 2-factor approximation for $ \cP_{d} $ in interval $ I $.


For any interval $ I $, and $ \eta > 0$ let $ \tilde{q}_{\cA_{d+1}, I}  $
be an $ \eta $ approximation to 
$  \hatq_{\cA_{d+1}, I} $, 
i.e. $  \tilde{q}_{\cA_{d+1}, I} $ satisfies
\[
\akkint{d+1}{I}{\tilde{q}_{\cA_{d+1}, I} -f} \le
\akkint{d+1}{I}{\hatq_{\cA_{d+1}, I} -f} +\eta.
\]


We first show that $  \tilde{q}_{\cA_{d+1}, I}  $ is bounded in its distance to 
any optimal degree-$d $ approximation $ q^{*}_{I} $. This fact is then used 
along with certain structural results on polynomials to provide a 2-factor
approximation to $ \cP_{d} $ in $ I $.
\begin{Lemma}
	\label{lem:tilde}
	The $ \ell_{1} $ distance between $  \tilde{q}_{\cA_{d+1}, I}  $ and any $ q \in \cP_{d}$,
	\[\loneint{I}{ \tilde{q}_{\cA_{d+1}, I} -q}	\le 
	2\loneint{I}{f-q} + 2\akkint{d+1}{I}{\hatf-f}+\eta.\]
\end{Lemma}
\begin{Proof}
	Note that
	\begin{align}
		\nonumber
		\loneint{I}{ \tilde{q}_{\cA_{d+1}, I} -q}
		&\overset{(a)}\le
		\akkint{d+1}{I}{ \tilde{q}_{\cA_{d+1}, I} -q}\\
		\nonumber
		&\le
		\akkint{d+1}{I}{ \tilde{q}_{\cA_{d+1}, I} -\hatf}+\akkint{d+1}{I}{ \hatf -q}\\
		\nonumber
		&\overset{(b)}\le
		\akkint{d+1}{I}{ \hat{q}_{\cA_{d+1}, I} -\hatf} +\eta +\akkint{d+1}{I}{ \hatf -q}\\
		\nonumber
		&\le 
		2\akkint{d+1}{I}{\hatf-q} +\eta\\
		\nonumber
		&\le 
		2\akkint{d+1}{I}{f-q} + 2\akkint{d+1}{I}{\hatf-f}+\eta\\
		\nonumber
		&\le 
		2\loneint{I}{f-q} + 2\akkint{d+1}{I}{\hatf-f}+\eta
	\end{align}
	where $ (a) $ follows since $ \tilde{q}_{\cA_{d+1}, I} -q \in \cP_{d}$,
	$ (b) $ follows from the property of the projection oracle described in Lemma~\ref{lem:proj} and $ (c) $ follows since $ \hatq_{\cA_{d+1},I} $,
	by definition refers to the degree-$ d $ polynomial that minimizes the $ \cA_{d+1} $
	distance to $ \hatf$ in $ I $.
\end{Proof}

We now establish a structural that bounds the integral of the absolute value 
of the derivative of a polynomial in terms of its $ \ell_{1} $ norm.
\begin{Lemma}
	\label{lem:poly}
	For any degree-$ d $ polynomial $p\in \cP_{d}$ and $x\in(-1, 1)$,
	\[
	\int_{-x}^{x}|p'(t)|\, dt
	%
	\,\le\,
	\frac{28(d+1)}{\sqrt{1-x^2}}
	%
	% \,\lesssim\,
	% \frac{d}{\sqrt{1-x^2}}
	%
	\int_{-1}^1|p(t)|\, dt.
	\]
\end{Lemma}
% \[
% |f(x)|\sqrt{1-x^2}
% \le
% d
% \int_ |f(t)| dt
% \]
%
\begin{Proof}
	%Here we describe a simplified proof that produces a larger 
	%constant, namely $8\pi d + 2\sqrt{2}(d+1)$. But the proof can be improved (by considering a different $f_d$) to obtain $3d+\text{\scriptsize $\mathcal{O}$}(1)$.
	%\\
	The case of $d=0$ is trivial. We give a proof for $d\ge 1$. Consider
	\[
	f_d(x)
	\, 
	\ed
	\,
	\frac{1}{\text{\normalsize $x$}}
	\sin(d \arcsin(x)).
	\]
	{\bf Claim 1}\quad $f_d$ is a degree-$(d\!-\!1)$ polynomial for odd $d$. E.g.,
	$
	f_5(x)
	=
	5 - 20 x^2 + 16 x^4.
	$
	\\
	{\bf Claim 2}\quad $\norm{f_d}_2\le \sqrt{\pi\,d}$,\,
	because
	\begin{align*}
		\norm{f_d}_2^2
		&=
		2\int_0^1
		\frac{\sin^2(d \arcsin(x))}{x^2}\,
		\,dx\le
		\int_{0}^{\frac{\pi}{2}}
		\frac{1-\cos(2d\theta)}{ \sin^2 \theta}\, d\theta
		=\pi\, d. 
	\end{align*}
	{\bf Claim 3}\quad
	$f_d(0) =d$ and  $f'_d(0)=0$. 
	\\
	Let $f(t)\ed p(t)\sqrt{1-t^2}$ and note that
	\begin{align*}
		\sqrt{1-x^2}\int_{-x}^x |p'(t)|\,dt
		&\le
		\int_{-1}^{1} |p'(t)|\sqrt{1-t^2}\,dt
		\le
		\int_{-1}^1 
		|f'(t)|\,dt
		+
		\int_{-1}^1 
		\frac{|t\, p(t)|}{\sqrt{1-t^2}} \,dt
	\end{align*}
	%
	Let $g_d(x) 
	\ed
	\sqrt{\frac{2}{\pi d}}
	\cdot f_{\frac{d}{2}}(x)$, then  $g_d(0)=\sqrt{\frac{d}{2\pi}}$ and $g'_d(0)=0$. Hence,
	\vspace{-.5em}
	\begin{align*}
		\frac{1}{2\pi}|f'(0)|
		&=
		\frac{1}{d}\,
		|f'(0)|\,
		g^2_d(0)
		{\overset{(a)}{\le}}
		2\max_{t} |f(t)|\,
		g^2_d(t)
		{\overset{(b)}{\le}}
		4d\int_{-1}^{1} |p(t)|\, g^2_d(t)\, dt,
	\end{align*}
	where $(a)$ and
	$(b)$ follow from the Bernstein's inequality since  
	$|p(t)|\sqrt{1-t^2}
	\le d\int_{-1}^1 |p(z)|dz$ for a degree$-d$ polynomial, and applying the inequality to $p(t)g_d^2(t)$ of degree $2d$. For $(a)$ we additionally observe that $g_d'(0)=0$ by construction.
	\\
	Equivalently, for
	$c\,\ed 8\pi $
	and $f_{\text{\tiny T}}(\theta)\ed f(\sin \theta)$,
	\begin{align*}
		|f_{\text{\tiny T}}'(0)|
		\,\le\,
		c\, d\int_{-\pi}^{\pi} |f_{\text{\tiny T}}(\theta)|\,g^2_d(\sin\theta)\,d\theta.
	\end{align*}
	The same reasoning also implies
	\[
	|f_{\text{\tiny T}}'(\alpha)|
	\le
	c\, d\int_{-\pi}^{\pi} |f_{\text{\tiny T}}(\theta+\alpha)|\,g^2_d(\sin\theta)\,d\theta
	=
	c\, d\int_{-\pi}^{\pi} |f_{\text{\tiny T}}(\theta)|\,g^2_d(\sin(\theta-\alpha))\, d\theta
	.
	\]
	Integrating both sides for $\alpha$ from $-\pi$ to $\pi$ yields
	\[
	\int_{-1}^1 
	|f'(t)| \,dt
	=
	\int_{-\pi}^{\pi} |f_{\text{\tiny T}}'(\alpha)|\, d\alpha
	\,{\overset{(a)}\le}\,
	c\,d\int_{-\pi}^{\pi} |f_{\text{\tiny T}}(\theta)|
	\,
	d\theta
	=
	c\,d\int_{-1}^{1} |p(t)|
	\,
	dt,
	\]
	where (a) follows since from Claim 2 and the definition of $g_d$, $\norm{g_d}_2\le 1$.
	%
	Finally, 
	for a proper $\tau\in(0, 1)$ of order $1/d^2$,
	\begin{align*}
		\int_{-1}^1 
		\frac{|t\,p(t)|}{\sqrt{1-t^2}}\,dt
		&\le 
		\int_{-1+\tau}^{1-\tau}\frac{|p(t)|}{\sqrt{1-t^2}}\,dt
		+
		2\max_t |p(t)|\int_{1-\tau}^{1}\frac{t}{\sqrt{1-t^2}}\,dt\\
		&{\overset{(a)}{\le} }
		\frac{\int_{-1}^1 |p(t)|\,dt}{\sqrt{2\tau-\tau^2}}
		+
		2\max_t |p(t)|\int_{1-\tau}^{1}\frac{t}{\sqrt{1-t^2}}\,dt\\
		&{\overset{(b)}{\le} }
		\frac{\int_{-1}^1 |p(t)|\,dt}{\sqrt{2\tau-\tau^2}}
		+
		2\sqrt{2\tau-\tau^2}\,
		(d+1)^2
		\int_{-1}^1|p(t)|\, dt\\
		&=
		{2\sqrt{2}}
		(d+1)\int_{-1}^1|p(t)|\, dt, 
	\end{align*}
	where $(a)$ follows by setting $1/\sqrt{1-t^2}$ to its greatest value, 
	$1/\sqrt{2\tau - \tau^2}$
	and $(b)$ follows from the Markov Brothers' inequality.
	Proof is complete by noting that $ 8\pi + 2\sqrt{2}< 28 $.
	\qedhere
\end{Proof}


We now define the partition $ \barJ(I, c_{1}, l) $ that takes advantage of Lemma~\ref{lem:poly}
. For simplicity we consider 
the interval $ [-1,1] $. The partition for $ I $ may be obtained by linearly translating 
$ \barJ([-1,1], c_{1}, l) $. 

For any $i\ge 1$ define the region 
$I_i\ed  [-(1-1/2^{i}), -(1-1/2^{i-1})]\cup[1-1/2^{i-1}, 1-1/2^i]$.
Further partition $I_i$ into $l (d+1)/2^{c_1\cdot i}$ sub-intervals of equal width. 
Thus each interval is of width $1/2^{i}\cdot 2^{c_1\cdot i}/(l(d+1)) = 1/(2^{(1-c_1)i}\cdot l(d+1))$.
Let this sub-partition of $ I_{i} $ be called $\barI_{i}(c_{1})= \barI_{i} $.
For an integer $ m\ge 1 $ denote the two terminal intervals as
$E_{m}\ed [-1,1]\setminus \Paren{\cup_{i=1}^m\barI_i}$.
For some $\epsilon>0$, let $m(\epsilon)\ed \log_2(l(d+1)^2/\epsilon)$. 
Observe that the length of the terminal region $ |E_{m(\epsilon)}|\le 2\epsilon/(l(d+1)^{2}) $.

Define $ \barJ = \barJ([-1,1], c_{1}, l) \ed  \cup_{i=1}^{m(\epsilon)}\barI_i \cup E_{m(\epsilon)}$. 
The total number of intervals in $ \barJ $ is given by
\[
\sum_{i=1}^{m(\epsilon)} |\barI_i| 
= \sum_{i=1}^{m(\epsilon)}  \frac{l(d+1)}{2^{c_1i}} 
\le 
\frac{l(d+1)}{2^{c_1}}
\cdot \frac{1}{1-2^{-c_1}}
=\frac{l(d+1)}{2^{c_1}-1}.
\]
Notice that the number of intervals is independent of $ \epsilon $, for example if $ c_{1} = 1/8 $,
$ \barJ(c_{1}) $ consists of $\le  12l(d+1)$  intervals. Define 
\[
k\ed \frac{l(d+1)}{2^{c_1}-1} .
\]
Lemma~\ref{lem:polyhist} bounds the $ \ell_{1} $ difference between 
any polynomial $ p\in \cP_{d} $ and its histogram on $ \barJ(I, c_{1}, l) $ denoted by 
$ \bar{p}_{\barJ(I, c_{1},l)} $.
\begin{Lemma}
	\label{lem:polyhist}
	Let $ p \in \cP_{d} $ be any degree-$ d$ polynomial in $ [-1,1] $. 
	Then for any $ l>0 $
	and $ 0<c_{1}<1/2 $, the histogram of $ p $ under the 
	partition $ \barJ = \barJ(I, c_{1},l) $ satisfies
	\[
	\loneint{I}{p-\barp_{\barJ}} \le \frac{\lone{p}}{l}
	{\frac{28}{1-2^{c_1-1/2}}}.
	\]
\end{Lemma}
\begin{Proof}
	Consider the interval $ I_{i} $ for $ i\in \{1\upto m\} $.
	Using Lemma~\ref{lem:poly}, we have
	\[
	\int_{I_i} |p'(z)|dz
	\le \int_{-\Paren{1-1/2^{i}}}^{\Paren{1-1/2^{i}}} |p'(z)|dz
	\le 
	\frac{28(d+1)\lone{p}}{(1-\Paren{1-1/2^{i}})^{1/2}}
	\le 
	2^{i/2}\cdot (d+1)\lone{p}.
	\]
	Since each interval in $ \barI_{i} $ is of width $ 1/ (2^{(1-c_1)i}\cdot l(d+1))$,
	the $\ell_1$ difference under the partition $\barI_i$ is given by
	\[
	\loneint{I_i}{p-\barp_{\barI_i}}
	\le 
	28\cdot 2^{(1/2+c)i}\cdot (d+1)\lone{p}.\frac{1}{2^{(1-c_1)i}\cdot l(d+1)}
	=
	\frac{28\cdot 2^{i(c+c_1-1/2)}\lone{p}}{l}.
	\]	
	Thus the total $ \ell_{1} $ difference 
	\begin{align*}
		\loneint{I}{p-\barp_{\barJ}}
		&=\sum_{i=1}^{m(\epsilon)} \loneint{I_{i}}{p-\barp_{\barI_{i}}} + \loneint{E_{m}}{p-\barp_{E_{m}}}\\
		&\le 
		\sum_{i=1}^{m(\epsilon)}
		\frac{28\cdot 2^{i(c_1-1/2)}\lone{p}}{l}
		+2p(E)\frac{\epsilon}{l(d+1)^2}\\
		&\overset{(a)}{\le }
		\sum_{i=1}^{m(\epsilon)}
		\frac{28\cdot 2^{i(c_1-1/2)}\lone{p}}{l}
		+4(d+1)^2\lone{p}\frac{\epsilon}{l(d+1)^2}\\
		&\overset{(b)}{\le }
		\frac{\lone{p}}{l}
		\Paren{\frac{28}{1-2^{c_1-1/2}}+\frac{\epsilon}4},
	\end{align*}
	where $(a)$ follows since $p\le (d+1)^2\lone{p}$ from the Markov Brothers' inequality and
	$(b)$ follows since $c_1<1/2$. Proof is complete by setting $ \epsilon $ to be arbitrarily small.
\end{Proof}

Inspired by Lemma~\ref{lem:polyhist}, given an interval $ I \subseteq \reals$, a partition $ 
\barI $ of $ I $, and 
an arbitrary integrable function $ h:I\rightarrow \reals $ we 
define the translation of a polynomial $ q\in \cP_{d} $ based on matching its mass
with $ h $ in intervals within $ \barI $.
\begin{Definition}
	\label{def:polytranslate}
	For a partition $ \barI $ of some interval $ I $ and an integrable function
	$ h:I\rightarrow \reals $ define the poly translation of $ q $ w.r.t. $ h$ as
	\[
	q_{h, \barI}(x)  \ed \sum_{I\in \barI}\mathbbm{1}_{x\in J}
	( q(x)+m_{I}), \text{ where for any interval $ J \subseteq \reals$, } 
	{m}_J \ed \int_{J} h(x)- q(x)dx.
	\]
\end{Definition}

Definition~\ref{def:polytranslate} along with Lemma~\ref{lem:polyhist}
implies Corollary~\ref{cor:polyhist} that bounds the difference between 
polynomials that are `translated' w.r.t. the same function.
\begin{Corollary}
	\label{cor:polyhist}
	Given polynomials $ p,q\in \cP_{d} $, an interval $ I $, and numbers $ l\ge 0, 1/2>c_{1}\ge0  $,
	for any integrable function $ h:I\rightarrow \reals $,
	\[
	\loneint{I}{p_{h,\barJ(I,c_{1},l)}
		-q_{h,\barJ(I,c_{1},l)}}
	\le 
	\frac{\loneint{I}{p-q}}{l}
	{\frac{28}{1-2^{c_1-1/2}}}.
	\]
\end{Corollary}
\begin{Proof}
	Let $ r \ed p-q$. Observe that by construction since the 
	mass of both $ p $ and $ q $ are made equal in each interval in $ \barJ(I, c_{1}, l) $,
	$
	\loneint{I}{p_{h,\barJ(I,c_{1},l)}-q_{h,\barJ(I,c_{1},l)}} 
	= \loneint{I}{r-r_{\barJ}}.
	$
	Proof follows by applying Lemma~\ref{lem:polyhist} to $ r $.
\end{Proof}

For simplicity denote $ \tilde{q} = \tilde{q}_{\cA_{d+1}, I} $. 
The $ \SPLIT $ estimate $ \hatq_{I}(x) $ is defined as.
\[
\hatq_{I}(x) \ed \tilde{q}_{\hatf, \barJ(I,c_{1},l)}.
\]
In other words $ \hatq_{I}(x) $ is obtained via adding a constant to 
$ \tilde{q}_{\cA_{d+1}, I}$ in
each interval to match its mass with $ \hatf $ in that interval.
$ \SPLIT $ is summarized in Algorithm~\ref{alg:SPLIT}.
\begin{algorithm}[h]
	\caption{$ \SPLIT $}
	\label{alg:SPLIT}
	\begin{algorithmic}
		\STATE {\bfseries Input:} $ X^{n} $, $ d $, $ I $, $ \tilde{q}_{\cA_{d+1}, I} $, $ c_{1} $, $ l $
		\STATE Denote $ \tilde{q}\gets  \tilde{q}_{\cA_{d+1},I}, \ \barJ \gets \barJ(I,c_{1},l)$
		\STATE {\bfseries Output:} $ \barJ, \tilde{q}_{\hatf, \barJ}$
	\end{algorithmic}
\end{algorithm}

Similarly define
\[
\barq_{I}(x) \ed \tilde{q}_{f, \barJ(I,c_{1},l)}.
\]
by adding a constant w.r.t. to $ f $. 
Recall that $ q^*_{I}\in \cP_{d} $ is one of the $ \OPT_{\cP_{d}}(f) $ achieving polynomials
in $ I $.
Denote $ {q}^{*} = {q}^{*}_{\cA_{d+1},I} $ and define 
\[
\barq^{*}_{I}(x) \ed q^{*}_{f, \barJ(I,c_{1},l)}.
\]
\begin{Lemma}
	Given an $ \eta $ approximate
	$ \cA_{d+1} $ minimizer to $ \hatf $ in $ I $, $  \tilde{q}_{\cA_{d+1}, I} $,
	and numbers $l\ge 0$, $1/2>c_1\ge 0$,
	$ \SPLIT $ returns a partition $ \barJ(I, c_{1}, l) $ and a piecewise $ \hatq_{I} $ such that
	\[
	\loneint{I}{\hatq_{I}-f}\le  \Paren{2+\frac{112}{l(1-2^{c_1-1/2})}}\OPT_{\cP_d, I}(f)+
	{\frac{28\Paren{2\akkint{d+1}{I}{\hatf -f}+\eta}}{l(1-2^{c_1-1/2})}}+\akkint{k}{I}{\hatf -f}.
	\]
\end{Lemma}


Thus the $ \ell_{1} $ distance from $ \hatq_{ I}$ to $f $ is bounded as
\begin{align}
	\nonumber
	\lone{\hatq_{I}-f}&\le \lone{\bar{q}^{*}-f}+\lone{\bar{q}_{I}-\bar{q}^*_{I}}+\lone{\hatq_{I}-\bar{q}_{I}}\\
	\nonumber
	&=
	\sum_{J\in \bar{J}}\loneint{J}{\bar{q}^*_{I}-f}+\lone{\bar{q}_{I}-\bar{q}^*_{I}}+\lone{\hatq_{I}-\bar{q}_{I}}\\
	\nonumber
	&\overset{(a)}{\le}  
	2\OPT_{\cP_d, I}(f)+\lone{\bar{q}_{I}-\bar{q}^*_{I}}+\lone{\hatq_{I}-\bar{q}_{I}}\\
	\nonumber
	&\overset{(b)}{\le}  
	2\OPT_{\cP_d, I}(f)+\lone{\bar{q}_{I}-\bar{q}^*_{I}}+\akkint{|J|}{I}{\hatf -f}\\
	\nonumber
	&\overset{(c)}{=}  
	2\OPT_{\cP_d, I}(f)+\lone{\bar{q}_{I}-\bar{q}^*_{I}}+\akkint{k}{I}{\hatf -f}\\
	\nonumber
	&\overset{(d)}{\le}  
	2\OPT_{\cP_d, I}(f)+\frac{\lone{\tilde{q}_{\cA_{d+1}, I}-q^{*}_{I}}}{l}
	{\frac{28}{1-2^{c_1-1/2}}}+\akkint{k}{I}{\hatf -f}\\
	\nonumber
	&\overset{(e)}{\le}  
	\Paren{2+\frac{56}{l(1-2^{c_1-1/2})}}\OPT_{\cP_d, I}(f)+
	{\frac{28\Paren{2\akkint{d+1}{I}{\hatf -f}+\eta}}{l(1-2^{c_1-1/2})}}+\akkint{k}{I}{\hatf -f},
\end{align}
where $(a)$ follows since $ \barq^* $ has the 
same probability mass as $f$ in each interval in $ \barJ $
and is parallel (therefore doesn't intersect) with the $\OPT_{\cP_1}(f)$ attaining $ q^{*}$,
$ (b) $ follows since by definition $ \hatq $ and $ \barq $ correspond 
to $ \hatq_{\cA_{d+1}} $  translated by the probability mass of $ \hatf $
and $ f $ in each interval in $ \barJ $, $(c)$ follows from the definition of $k$,
$ (d) $ follows from Corollary~\ref{cor:polyhist} since by definition
$ \barq_{I}(x) = \tilde{q}_{f, \barJ(I,c_{1},l)} $ and $ \barq^{*}_{I}(x) = q^{*}_{f, \barJ(I,c_{1},l)} $ 
(recall $ \tilde{q}=\tilde{q}_{\cA_{d+1}, I} $ and $q^{*} = q^{*}_{I}$)
and $ (e) $ follows from Lemma~\ref{lem:tilde}.


==> interactive2.tex <==
\ignore{-.5em}
\section{The Compare and Stitch Routines}
\label{sec:stitch}
\ignore{-.25em}
This section presents $ \STITCH $ and $ \MERGE $, the main routines 
of $ \SURF $. For any contiguous collection of intervals $\barI$, let $ \hatf_{\barI,\EQ} $ 
be the piecewise polynomial estimate consisting of $ \hatf_{I, \EQ} \in \cP_d$
given by $ \EQ $ in each $ I\in \barI $. The key idea in 
$ \SURF $ is to separate interval partitions into a binary hierarchy, effectively 
allowing a comparison of all the $ \Omega(n^{c})$ (for any $ c>0 $) 
estimates corresponding to the different interval partitions, 
but by using only $ \tilde{\cO}(n) $ comparisons. 
\ignore{-.5em}
\subsection{Notation}
\ignore{-.25em}
\ignore{Let $ \barhatp_0 \ed (1/n\upto 1/n) $
and recall that its interval partition is given by
$ \barI_{\barhatp_0} $.
In this case, intervals in $ \barI_{\barhatp_0} $
are defined simply by pairs of consecutive samples.}

Recall that $ n $ here a power of $ 2 $ 
and define the integer
\ignore{-.5em}
\[D \ed \log_{2} n. 
\ignore{-.5em}\]
An empirical distribution, $ \barhatp \in \Delta_{\mathrm{emp,n}} $,
is called a \emph{binary} distribution if each of its probability values 
are of the form $ 1/2^d $, for some integer 
$0\le d\le D$. The corresponding interval partition, 
$ \barI_{\barhatp} $, is said to be 
a \emph{binary partition}.
\begin{align*}
\Delta_{\mathrm{bin,n}}
&\ed 
\{\barhatp\in \Delta_{\mathrm{emp,n}}
:\forall \hatp\in\barhatp, \\
&\phantom{\ed\Big (}\hatp=1/2^{\nu(\hatp)}, 0\le \nu(q)\le D, \ 
\nu(q)\in \mathbb{Z}\}.
\end{align*}
For example $ \barhatp=(1)$, $\barhatp=(1/2,1/4,1/4)$,  
$\barhatp=(1/4,1/8,1/8,1/2) $ are binary
distributions. Similarly, $\baru{n} = \baru{2^{\log n}}$
is also a binary distribution since $ n $ here is 
a power of 2 (assume $ n\ge 8 $ so that they 
are all in $\Delta_{\textrm{emp,n}}$).
\begin{Lemma}
\label{lem:binarycomp}
For any empirical distribution
$ \barhatp \in \Delta_{\mathrm{emp,n}}$, 
there exists $  \barhatp' \in \Delta_{\mathrm{bin,n}}$ 
such that
\[
\lone{\starf_{\barI_{\barhatp'}}-f} \le
\lone{\starf_{\barI_{\barhatp}}-f}, \
\sum_{\hatp \in \barhatp'}
\epsilon\sqrt{\hatp}
\le
\sum_{\hatp\in \barhatp}
\frac{1}{\sqrt{2}-1}\epsilon\sqrt{\hatp},
\]
where $ \starf_{\barI} $ is the piecewise 
polynomial closest to $ f $ on $ \barI $.
\end{Lemma}
Lemma~\ref{lem:binarycomp} shows that $\Delta_{\mathrm{bin,n}}$ retains
most of the approximating power of $\Delta_{\mathrm{emp,n}}$. In particular, that
for any $ \barhatp \in \Delta_{\mathrm{emp,n}}$, there exists a binary distribution $\barhatp' \in \Delta_{\mathrm{bin,n}}$ such that
$ \barI_{\barhatp'} $ has
a smaller bias than $ \barI_{\barhatp} $, while its
deviation under the 
concentration event, $ \cQ_{\epsilon} $,
is larger by less than a factor of $ 1/(\sqrt{2}-1) $.

For a fixed $ \barp\in \Delta_{\mathrm{bin,n}}$,
let $\Delta_{\mathrm{bin,n}, \le \barp}$ be the 
set of binary distributions such that for any 
$\barhatp \in \Delta_{\mathrm{bin,n}, \le \barp}$,
each $ I_1\in \barI_{\barhatp} $ is contained 
in some $I_2 \in \barI_{\barp} $.  
\begin{equation}
\label{eqn:nestbin}
\Delta_{\mathrm{bin,n}, \le \barp } \ed 
\{\barhatp\in \Delta_{\mathrm{bin,n}}
:\forall I_1 \in \barI_{\barhatp}, \
\exists I_2 \in \barI_{\barp}, \
I_1\subseteq I_2
\}.
\end{equation}
For example if $ \barp=(1/2,1/4,1/4) $ is the 
binary distribution, $ (1/4,1/4,1/8, 1/8,1/4), 
(1/2,1/4,1/8,1/8) \in \Delta_{\mathrm{bin,n},\le \barp}$, whereas
$ (1/2,1/2) \notin  \Delta_{\mathrm{bin,n},\le \barp} $. 

Similarly, let $\Delta_{\mathrm{bin,n}, \ge \barp}$ 
consist of binary distributions such that
for any $\barhatp \in \Delta_{\mathrm{bin,n}, \ge \barp}$,
each $I_1\in \barI_{\barp} $ is contained in 
some $I_2 \in \barI_{\barhatp} $. 
\[
\Delta_{\mathrm{bin,n}, \ge \barp } \ed 
\{\barhatp\in \Delta_{\mathrm{bin,n}}
:\forall I_1 \in \barI_{\barp}, \
\exists I_2 \in \barI_{\barhatp}, \
I_1\subseteq I_2
\}.\]
For example,  if $ \barp=(1/2,1/4,1/4) $, then
$ (1/2,1/2) \in \Delta_{\mathrm{bin,n},\ge \barp},$
but $ (1/2,1/8,1/8,1/4) \notin \Delta_{\mathrm{bin,n},\ge \barp}.$
A complimentary relationship exists between
$ \Delta_{\mathrm{bin,n},\le \barp} $ and 
$\Delta_{\mathrm{bin,n},\ge \barp}$.
For any $ \barp_1, \barp_2 \in
\Delta_{\textrm{bin,n}}$,
$ \barp_1\in  \Delta_{\mathrm{bin,n},\le \barp_2}$ $ \Leftrightarrow $
$  \barp_2 \in \Delta_{\mathrm{bin,n},\ge \barp_1}$.
\ignore{-.5em}
\subsection{The $\STITCH$ Routine}
\ignore{-.25em}
$ \STITCH$ receives as input, $ X^{n-1} $ and 
parameters $ d $, $\alpha$, $ \epsilon $.

The routine operates in $i\in\{1\upto D\} $ steps.
Define $ D(i)\ed D-i$ and let
\[ \bar{u}_i \ed \left(\frac{1}{2^{D(i)}}\upto \frac{1}{2^{D(i)}}\right), \
\barI_{\bar{u}_i} =(I_{\bar{u}_i,1}\upto I_{{\bar{u}_i}, 2^{D(i)}}).\]
%where the latter denotes the interval partition under $ \bar{u}_i $.
Initialize $\barhatp_0\gets  \baru{n}$. 

Start with $ i =1  $ and assign $ \barhats \gets \barhatp_{i-1}$.
In each step, the routine maintains this
$\barhats = \barhatp_{i-1}\in \Delta_{\mathrm{bin,n},\le \bar{u}_i}$.
This can be seen from the initialization above
for $ i=1 $ since $ \bar{u}_1 = (2/n\upto 2/n) $, 
and verified for $ i>1 $. Thus, using $ \barI_{\bar{u}_{i}} $, 
we may separate
\[
\barI_{\barhats}
=(\barI_{\barhats,1}\upto \barI_{\barhats,2^{D(i)}}),\
\barhats=(\barhats_1\upto\barhats_{2^{D(i)}}),
\]
where for each $ j\in\{1\upto 2^{D(i)}\} $,
$\barI_{\barhats,j}\subseteq \barI_{\barhats}$
are intervals in $ \barI_{\barhats} $ whose union 
gives $ I_{\bar{u}_i,j}\in \barI_{\bar{u}_i} $. 
Let $\barhats_j\in \barhats$ denote the empirical probabilities in $ \barhats $
corresponding to intervals in $ \barI_{\barhats,j}$.
Notice that the sum of all probabilities in $ \barhats_j $, 
$\sum_{\hats\in \barhats_j}\hats = 1/2^{D(i)} $.
Therefore the scaled $ 2^{D(i)}\barhats_j $
is an empirical distribution.
For brevity, let the polynomial estimate
output by $ \EQ $ on $ I_{{\bar{u}_i},j} $,
be denoted by
\[ \hatf_{I_j}\ed \hatf_{I_{{\bar{u}_i},j},\EQ}. \]
Starting with $ j=1 $, invoke $ \MERGE $ with arguments, 
the polynomial estimate $ \hatf_{I_j} $,
intervals $ \barI_{\barhats,j} $ and the empirical
distribution $ 2^{D(i)}\barhats_j $, samples 
$ X^{n-1}_{i,j}
\subseteq X^{n-1} $ that lie in $ I_{\bar{s},j} $, and parameters $ d $,
\[\gamma \ed 
\alpha\cdot r_d \cdot \epsilon \sqrt{d+1}.
\]
This parameter, $\gamma$, is used to
tune the bias-variance trade-off. 
As will be shown subsequently, 
if $ \gamma \rightarrow\infty $,
$ \barI_{\barhats,j} $ will be merged, resulting in 
an estimate with a larger bias but smaller variance.
A small $ \gamma $ has the opposite effect.

If $ \MERGE(\hatf_{I_j}, \barI_{\barhats,j}, 
2^{D(i)}\barhats_j, X^{n-1}_{i,j},d,\gamma)\le 0 $,
merge $\barI_{\barhats,j}  $ 
into a single interval $ I_{\bar{u}_i,j} $. Accomplish this by
updating $\barhats_j$ to a unitary value, 
its sum, ($ 1/2^{D(i)}$).  
Otherwise, maintain $ \barhats $ as is.
Increment $j$ within the range 
$\{1 \upto 2^{D(i)}\}$ and repeat this procedure.

After the entire run in $ j $ is complete, 
update $\barhatp_i\leftarrow \barhats$.
If $ D(i)=D-i>0$, increment $i$ and 
repeat the same steps.
Otherwise, if $ D(i)=0$ or in other words if $ i=D$, 
$ \STITCH $,  
and in turn, $ \SURF $ outputs the piecewise 
estimate on $ \barI_{\barhatp_{D}} $, i.e. 
$ \hatf_{\text{SURF}}   =\hatf_{\barI_{\barhatp_{D}},\EQ } $.

At each step $ i\in \{1\upto D\} $, $ \STITCH $ calls 
$ \MERGE $ on $2^{D(i)} $ intervals,
each consisting of $ 2^i $ samples. 
Thus each step of $ \STITCH $ takes
$ \cO(2^{D(i)}\cdot (d^{\tau}+\log (2^i)) \cdot 
2^i) = \cO((d^{\tau}+\log n )2^D)$ time. 
The total time complexity is therefore 
$\cO((d^{\tau}+\log n )2^D D) = \cO((d^{\tau}+\log n)n\log n ) $.

\begin{algorithm}[tb]
   \caption{$ \STITCH $}
   \label{alg:STITCH}
\begin{algorithmic}
   \STATE {\bfseries Input:} $ X^{n-1} $, $ d $, $\alpha$, $ \epsilon $
   \STATE Initialize $D= \log n, \barhatp= \baru{n}$
   \FOR{$i=1$ {\bfseries to} $D$}
	\STATE $ D(i)\gets D-i  ,\ \barhats\gets \barhatp$
%	\STATE $ \barI_{\barhats} \ed(\barI_{\barhats,1}\upto \barI_{\barhats,2^{D(i)}}),\ {\barhats} \ed ({\barhats_1}\upto \barhats_{2^{D(i)}})$
    \FOR{$j=1$ {\bfseries to} $2^{D(i)}$}
	\IF{$ \MERGE(\hatf_{I_j},   \barI_{\barhats,j},  2^{D(i)}\barhats_j , X^{n-1}_{i,j},d, \gamma)$ 
	$\le 0$}
   \STATE $ \barhats_j \gets (1/2^{D(i)})$
   \ENDIF
	\ENDFOR
	\STATE $ \barhatp \gets \barhats $
   \ENDFOR
\STATE {\bfseries Output:} $ \hatf_{\barI_{\barhatp},\EQ} $
\end{algorithmic}
\end{algorithm}
\ignore{-.5em}
\subsection{The $\MERGE$ Routine}
\ignore{-.25em}
$ \MERGE $ receives as input, a function $ \hatf $, 
an interval partition $ \barI \ed \barI_{\barhats} $ 
and the corresponding empirical 
distribution $ \barhats $, samples $ X^{m} $ that lie in $ \barI $, 
and parameters $ d $, $ \gamma $.

\ignore{Notice that the number of samples within $ I $
is given by $ \sum_{s\in\barhats}s\cdot n $.
While $ \barhats $ forms a sub-distribution in general,
WLOG assume it is a distribution, 
implying $ I $ has all $ n-1 $ samples. }

Fix a $ \barp \in \Delta_{\mathrm{bin,m},\ge \barhats} $,
and consider the piecewise polynomial estimate 
on $ \barI_{\barp} $, $ \hatf_{\barI_{\barp},\EQ} $. Define
\begin{equation}
\label{eqn:thr}
\del_{\barI_{\barp}}(\hatf)
\ed
\loneint{\barI_{\barp}}{\hatf_{\barI_{\barp},\EQ}
	-\hatf},\
\thr_{\barp, \gamma}\ed 
\sum_{p\in \barp}
\gamma \sqrt{p}.
\end{equation}
 $ \MERGE(\hatf) $ returns 
$ \lemerge_{\barI_{\barhats},\gamma}(\hatf) $, 
the largest difference between $ \del_{I_{\barp}}(\hatf) $
and $ \thr_{\barp,\gamma} $ across all
$ \barp\in \Delta_{\mathrm{bin,m}, \ge \barhats } $,
\[
\lemerge_{\barI_{\barhats},\gamma}(\hatf)
\ed
\max_{\barp \in \Delta_{\mathrm{bin,m}, \ge \barhats }}
\del_{\barI_{\barp}}(\hatf)-\thr_{\barp, \gamma}.
\]
The quantity, $ \del_{\barI_{\barp}}(\hatf) $ acts as a proxy for the increment 
in bias that results if the piecewise estimate
$ \hatf_{\barI_{\barp},\EQ} $ is merged into $ \hatf $, while 
$ \thr_{\barp, \gamma} $ accounts for the deviation in 
$\hatf_{\barI_{\barp},\EQ} $ under $ \cQ_{\epsilon} $.
Notice that for any 
$\barp \in \Delta_{\textrm{bin,m}, \ge \barhats} $,
$ \thr_{\barp, \gamma} \le \thr_{\barhats, \gamma}$.
Thus $ \lemerge_{\barI_{\barhats},\gamma}(\hatf)
\le 0 $ 
if the decrease in deviation under $ \barI = \barI_{\barhats} $ is larger 
than the increased bias under any candidate $ \barI_{\barp} $. 
This in turn signals $ \STITCH $ to merge $ \barI $.

It may be shown that if $ \barhats = \baru{m} $,
the cardinality, $ |\Delta_{\mathrm{bin,m}, \ge \barhats }|  
= \Omega(m ^c)$ for any $ c>0 $. Therefore,
naively evaluating $ \del_{I_{\barp}}(\hatf)-\thr_{\barp,\gamma} $ over each
$\barp \in \Delta_{\mathrm{bin,m}, \ge \barhats } $ 
incurs a worst case time complexity that is 
super-linear in $ m $. Instead, $ \MERGE $ uses
a simple divide-and-conquer procedure that computes 
$ \lemerge_{\barI_{\barhats},\gamma}(\hatf) $
in time $ \cO((d^{\tau}+\log m)m)$.

To describe this, notice that
if $ \barI_{\barhats} $ is a singleton $ (I) $, then $ \barhats = (1)$, implying
$\Delta_{\mathrm{bin,m}, \ge \barhats }= \{(1)\}$. 
In this case, obtain $ \hatf_{I, \EQ} \in \cP_d$
and return 
\[\lemerge_{\barI_{\barhats},\gamma}(\hatf)=
\del_{\barI_{(1)}}(\hatf)-\thr_{(1),\gamma}=
\loneint{\barI_{(1)}}{\hatf_{I, \EQ} - \hatf}-\gamma\sqrt{1}.
\]

If $ \barI_{\barhats} $ is non singleton or 
$ \barhats \neq (1) $, any 
$ \barp \in \Delta_{\mathrm{bin,m}, \ge \barhats } \setminus\{ (1)\}$ 
may be split into two sub-distributions, $ \barp_1 $, 
$ \barp_{2} $ that each sum to $1/2$. For example,
if the particular $\barp = (1/4,1/4,1/8,1/8,1/4)$,
it may be split into $\barp_1 = (1/4,1/4)$ and 
$ \barp_2 = (1/8,1/8,1/4) $. The corresponding
interval partition is also split into 
$\barI_{\barp} =  (\barI_{\barp_{1}},\barI_{\barp_{2}})$.
Since $ \barhats \neq (1)$, 
this may also be similarly split 
into $ \barhats_1 $ and $\barhats_2$. 
As a consequence, $ \barI_{\barhats}$ is also cleaved
into $ (\barI_{\barhats_1}, \barI_{\barhats_2}) $ 
corresponding to $ \barhats_1 $ and $\barhats_2$. 
Using this observation,
\begin{align*}
&\max_{\barp \in \Delta_{\mathrm{bin,m}, \ge \barhats } , \ 
\barp \neq (1)}
\del_{\barI_{\barp}}(\hatf)-\thr_{\barp,\gamma}\\
&=\max_{\barp \in \Delta_{\mathrm{bin,m}, \ge \barhats } , \ 
\barp \neq (1)}
\del_{\barI_{\barp_1}}(\hatf)-\thr_{\barp_1,\gamma}\\
&\phantom{\max_{\barp \in \Delta_{\mathrm{bin,m}, \ge \barhats } , \ 
\barp \neq (1)}}+\del_{\barI_{\barp_2}}(\hatf)-\thr_{\barp_2,\gamma}\\
&=\max_{\barp_1 \in \Delta_{\mathrm{bin,m}/2, \ge 2\barhats_1 } }
\del_{\barI_{\barp_1}}(\hatf)-\thr_{\barp_1,\gamma/\sqrt2}\\
&\phantom{=}+\max_{\barp_2 \in \Delta_{\mathrm{bin,m}/2, \ge 2\barhats_2 }} 
\del_{I_{\barp_2}}(\hatf)-\thr_{\barp_2,\gamma/\sqrt2}\\
&=\lemerge_{\barI_{2\barhats_1},\gamma/\sqrt2}(\hatf)
+\lemerge_{\barI_{2\barhats_2},\gamma/\sqrt2}(\hatf),
\end{align*}
where $ 2\barhats_1 $, $ 2\barhats_2 $ are the 
normalized variants of $ \barhats_1 $, $ \barhats_2 $, 
and $ \gamma $ is scaled by $ 1/\sqrt{2} $ to accommodate 
for this scaling. By evaluating
$\lemerge_{\barI_{2\barhats_1},\gamma/\sqrt2}
(\hatf) $,
$\lemerge_{\barI_{2\barhats_1},\gamma/\sqrt2}
(\hatf)$ separately, and then comparing their sum with
$ \del_{\barI_{(1)}}(\hatf)-\thr_{ (1),\gamma} $,
we allow for a recursive computation of 
$\lemerge_{\barI_{\barhats},\gamma}(\hatf) $.

Let $ X_{1}^{m} $ and $ X_2^{m}$ denote
the samples in $ \barI_{\barhats_1} $ and $ \barI_{\barhats_2} $ respectively.
Using these arguments, call $ \MERGE $ on 
$ \barI_{\barhats_1}, \barhats_{1} $ and 
$ \barI_{\barhats_2}, \barhats_{2} $,
return the maximum as shown in Algorithm~\ref{alg:COMP}.

Now $ \del_{\barI_{(1)}}(\hatf)-\thr_{ (1),\gamma} $
is calculated by obtaining $ \hatf_{I, \EQ} \in \cP_d$ 
from $ \EQ $. Since $ I $ has $ m $ samples, from 
Theorem~\ref{thm:polyblack}, this takes
$ \cO(m+d^{\tau}) $ time. Further, notice that since 
both $ \barhats_1 $ and $ \barhats_2$
sum to $ 1/2 $, the split $ \barI_{\barhats}=
(\barI_{\barhats_1},\barI_{\barhats_2}) $ occurs along
the median of $ X^{m} $. Thus $ \barI_{\barhats_1} $
and $ \barI_{\barhats_2} $ has at most half the
number of samples, $ m/2 $, and the time
complexity of $ \MERGE $, $ T(m) $, is captured by
\[T(m)\le 2T(m/2)+\cO(m+d^{\tau}),\]
implying $ T(m) = \cO((d^{\tau}+\log m)m) $.

\begin{algorithm}[tb]
   \caption{$ \MERGE $}
   \label{alg:COMP}
\begin{algorithmic}
   \STATE {\bfseries Input:} 
$ \hatf $, $ \barI_{\barhats} $,  $ \barhats $, $ X^{m} $, $ d $,$\gamma$
	\STATE $ I\gets \cup \barI_{\barhats}, \
	\lemerge\gets 
	\del_{I}(\hatf) -\thr_{\barhats,\gamma}$
	\IF{$ |\barI|=1 $}
	\STATE {\bfseries Return}: $ \lemerge $
	\ELSE
	\STATE {\bfseries Return}: $\max\{ \lemerge,\MERGE(\hatf, \barI_{\barhats_1},
 2\barhats_{1} ,  X_{1}^{m} ,d,\gamma/\sqrt{2} )$
	\STATE $ \phantom{\max\{ v,}+\MERGE(\hatf,\barI_{\barhats_2},
 2\barhats_{2} ,  X^{m}_{2} ,d, \gamma/\sqrt{2})\}$
	\ENDIF 
\end{algorithmic}
\end{algorithm}

Lemma~\ref{lem:master} shows that under 
$ \cQ_{\epsilon} $, 
$ \hatf_{\SURF }$ is within a constant 
factor of the best piecewise polynomial approximation 
over any binary partition, plus its deviation in probability 
under $ \cQ_{\epsilon} $ times $ \cO(\sqrt{d+1}) $.
\begin{Lemma}
\label{lem:master}
Given samples $ X^{n-1}\sim f $, for some $ n $ that 
is a power of $ 2 $, degree $ d\le 8 $ and
the threshold $ \alpha > 2$, $ \SURF$ 
outputs $ \hatf_{\text{SURF}} $ in time 
$ \cO((d^\tau+\log n)n\log n) $ such that under event 
$ \cQ_{\epsilon} $,
\begin{align*}
&\lone{\hatf_{\text{SURF}}-f}\\
&\le
\min_{\barp \in \Delta_{\mathrm{bin,n}}}
\sum_{I \in \barI_{\barp}} \left(
\frac{(r_d+1)\cdot \alpha}{\alpha-2}\cdot 
\inf_{\poly \in \cP_d}\loneint{I}{\poly-f}\right.\\
&\phantom{\le
\min_{\barhatp \in \Delta_{\mathrm{bin,n}}}
\sum_{I \in \barI_{\barp}} \left(\right.
}
\left.\ +\frac{r_d\cdot (\alpha\sqrt2+\sqrt{2}-1)}{\sqrt{2}-1}
\epsilon \sqrt{(d+1)\hatp_{I}}\right),
\end{align*}
where $ q_I $ is the empirical mass under interval $ I $,
$ r_d $ is the constant corresponding
to the $ \EQ $ routine in 
Theorem~\ref{thm:polyblack}.
\end{Lemma}
Lemma~\ref{lem:master}, along with Lemma~\ref{lem:binarycomp} 
that establishes the approximating power 
of binary partitions proves 
Theorem~\ref{thm:interhistopt}.

==> interval.tex <==
\section{Intervals and Partitions}
\label{sec:interval}
\subsection{Intervals}
For $n\ge1$, let $X^{(n-1)}\ed \ordst{X}{1}\upto \ordst{X}{n-1}$ 
be the increasingly-sorted values of $X^{n-1}$.
%Define $\ordst{X}{0}=-\infty$, $\ordst{X}{n}=\infty$.
For integers $0\le a<b\le n$, these samples
define intervals on the real line $\reals$,
\[
I_{a,b}
\ed
\begin{cases}
(-\infty,\ordst{X}{b}) &\text{if} \ a=0,\\
[\ordst{X}{a},\ordst{X}{b}) &\text{if} \ 0<a<b<n,\\
[\ordst{X}{a},\infty) &\text{if} \  b=n.\\
\end{cases}
\ignore{-0.5em} 
\]
The \emph{interval-} and \emph{empirical-probabilities} are
\ignore{-0.5em} 
\[
\intp_{a,b} \ed \int_{I_{a,b}}dF, \ \text{and }\
\hatp_{a,b}\ed \frac{b-a}{n}.
\ignore{-0.5em} 
\] 
For any $ 0\le a<b\le n $, $ I_{a,b} $ forms a 
\emph{statistically equivalent} block~\cite{tukey47}, wherein
$\intp_{a,b}\sim\Beta(b-a,n-(b-a))$ regardless of $ f $, and $ \intp_{a,b} $ concentrates to $ \hatp_{a,b} $.
\begin{Lemma}
\label{lem:singleconc}
For any $ 0\le a<b\le n $, $\epsilon\ge 0$,
\ignore{-.5em}
\[
\Pr[|\intp_{a,b}-\hatp_{a,b}|\ge \epsilon\sqrt{\hatp_{a,b}}]
\le 
e^{\frac{-(n-1)\epsilon^2}{2}}
+e^{\frac{-(n-1)\epsilon^2 \hatp_{a,b}}
{2(\hatp_{a,b}+\epsilon\sqrt{\hatp_{a,b}})}}.
\ignore{-.75em}
\]
\ignore{-.75em}
\end{Lemma}
%
We extend this concentration from one interval to many. 
For a fixed $ \epsilon >0 $, let 
$ \cQ_{\epsilon} $ be the event that
\[
\forall \ 0\le a<b\le n ,\ 
|\intp_{a,b}-\hatp_{a,b}|\le\epsilon\sqrt{\hatp_{a,b}}.
\]
\begin{Lemma}
\label{lem:multconc}
%add $ \epsilon\ge  1/\sqrt{n}$ and change statment
%for camera ready
For any $n\ge 128$ and $ \epsilon\ge 0 $,
\[
P[\cQ_{\epsilon}]\ge 1- \frac{n(n+1)}{2}
\left(e^{\frac{-(n-1)\epsilon^2}{2}}
+e^{-\frac{(n-1)\epsilon^2
}{2(1+\epsilon\sqrt{n})}}\right).
\]
%for camera ready change
\end{Lemma}
\ignore{-.75em}
Notice that $ \cQ_{\epsilon} $ refers to a stronger concentration event
that involves $ \sqrt{\hatp_{a,b}} $ $ \forall 0\le a<b\le n $ and 
standard VC dimension based bounds cannot be 
readily applied to obtain Lemma~\ref{lem:multconc}.
\ignore{-.5em}
\subsection{Partitions}
\ignore{-.25em}
A collection of countably many disjoint intervals whose 
union is $\reals$ is said to be a partition of $\reals$.
A distribution $ \barhatp $, consisting
of interval empirical probabilities is called an \emph{empirical distribution}, 
or that each probability in $ \barhatp $ is a multiple of $ 1/n $. 
The set of empirical probabilities, $ \Delta_{\mathrm{emp,n}} $, is defined as
\begin{equation}
\label{eqn:empiricaldist}
\Delta_{\mathrm{emp,n} } \ed 
\{\barhatp\in \Delta: 
\forall \hatp \in \barhatp, \
\hatp=\nu(\hatp)/n, \
\nu(\hatp)\in \mathbb{Z} \}.
\end{equation}
Since each $ \hatp\in \barhatp \in \Delta_{\mathrm{\mathrm{emp,n}}} \ge 1/n$,
$ \barhatp $ may be split into its finitely many probabilities as
$\barhatp=(\hatp_1\upto\hatp_k)$. 
For $1\le i\le k$, let $\hatcump_{i}\ed\sum_{j=1}^{i-1}\hatp_j$.
We use an empirical distribution to define an 
\emph{interval partition} as follows:
\begin{align}
\nonumber
\barIp{\barhatp}
&\ed
(I_{\hatcump_1n,(\hatcump_1+\hatp_1)n},
I_{\hatcump_2n,(\hatcump_2+\hatp_2)n}
\upto\\
\label{eqn:emppart}
&\phantom{\ed(}
I_{\hatcump_kn,(\hatcump_k+\hatp_k)n}).
\end{align}
%
These are the intervals that contain the first  increasingly sorted $\hatp_1n$ samples, 
the next $\hatp_2n$ samples and so on. For example
$I_{\hatcump_1n,(\hatcump_1+\hatp_1)n}
=I_{0,\hatp_1n}
=(-\infty,\ordst{X}{\hatp_1n})$ is 
the interval with the smallest $\hatp_1n$
samples, 
$I_{\hatcump_2n,(\hatcump_2+\hatp_2)n}
=I_{\hatp_1n,\hatp_2n+\hatp_1n}
=[\ordst{X}{\hatp_1n},\ordst{X}{(\hatp_1+\hatp_2)n})$ is 
the interval with the next $\hatp_2n$
samples, so on, and
\begin{align*}
I_{\hatcump_kn,(\hatcump_k+\hatp_k)n}
&=I_{\sum_{j=1}^{k-1}\hatp_jn,\hatp_kn+\sum_{j=1}^{k-1}\hatp_jn}\\
&=I_{\sum_{j=1}^{k-1}\hatp_jn,n}
=[\ordst{X}{1+\sum_{j=1}^{k-1}\hatp_jn},\infty)
\end{align*}
is the interval with the largest $\hatp_kn$ samples.


==> limitation.tex <==
\subsection{Limitations of $\cA_{d+1}$ minimization}
\label{sec:limitations}
In this section we show the limits of $ \cA_{d+1} $ 
distance minimization. We show that 
w.r.t. to the class $ \cP_{1} $, $ \cA_{k} $
minimization incurs an $ \OPT $ approximation factor $ > 2 $.

For simplicity consider the interval $I= [0,1] $ and for an integrable 
$ g:\reals\rightarrow \reals $, integers $ d\ge 0, t, k>1 $ denote the 
$ t $-piece degree-$ d $ minimizer to $ g $
$g_{\cA_{k}, t ,d}= g_{\cA_{k}, t,d, I}  $.

We now describe a construction of a 
distribution class that is indistinguishable using $ n $ samples with an 
arbitrarily high probability.
Consider a density $ g\in [0,1] $. Let $ \cG $ denote the set of 
non-negative continuous functions in $ [0,1] $
and let $ \cG_{g}\subseteq \cG $ be the subset $ \le g $, i.e. 
\[
\cG_{g} \ed \{g' \in \cG : g' \le g\}.
\]
We denote $ \cG_g$ as the \emph{lower envelope} class corresponding to $g$. 

For any positive integer $ m $ and $ w\in \reals^{+} $
let $ \cD_{m,w} $ be the set of functions composed of 
$ m $ dirac spikes in $ [0,1] $ where each spike is of weight $ w $.
Fix a $ g'\in \cG_{g}$, $ 0<\delta\le 1$ and suppose $ m>n^2/\delta $. Define
\[ 
w(g, g')=   \frac{\int_{0}^{1}g(z)-g'(z)dz}{m},
\]
\[
\cD_{g, g',m, \delta} 
\ed \Bigg\{
g''\in \cD_{m, w(g,g')}: \forall I\subseteq [0,1], \ \int_{I} g''(z) dz\in \int_{I} g(z)-g''(z) dz\pm 5/m 
\Bigg\}
\]
In other words each distribution in $ \cD_{g, g',\delta,m} $ has its mass nearly identical to 
that of $ g-g' $. We define the envelope class as
\[
\cC_{g,\delta,m} = \{g' + g'', \ g' \in \cG_{g}, \ g''\in \cD_{g, g',\delta,m}\}.
\]

For any $ m>n/\delta^{2} $,
consider two distributions $ g_{1}, g_{2} \in \cC_{g,m,\delta}$. 
It can be shown that $ g_{1} $ and $ g_{2} $ cannot be distinguished 
using  $n$ samples w.p.  $ \ge 1-\delta$ from standard collision arguments. 


We first show that the $ \cA_{2} $ minimizer to $ \hatf $ 
over the class of linear polynomials, $\hatf_{\cA_{2}, 1 ,1} $
suffers an $ \OPT $ approximation factor $ >2 $.

\begin{Lemma}
	Let $ \hatf $ be the empirical distribution corresponding to $ X^{n}\sim f $.
	Let $ \hatf_{\cA_{2}, 1 ,1} $  be the linear polynomial that minimizes
	the $ \cA_{2} $ distance to $ \hatf $. Then, there exists a distribution $ f \in \cC_{g,m,\delta }$ such with probability $\ge 1-\delta$
	\[
	\lone{\hatf_{\cA_{2}, 1 ,1}-f}\ge 2.136\OPT_{\cP_{1}}(f)-\frac{10}{m}.
	\]
\end{Lemma}
\begin{Proof}
	Consider the envelope $g$ given by 
	the distribution shown in Figure~\ref{fig:1}. 
	\begin{figure}[h]
		\centering
		\includegraphics[scale=0.7]{fig1}
		\caption{Single piece envelope. For any $ 0\le \delta<1 $,
			$ \cA_{2} $ minimizer to 
			$ \cC_{g,\delta,m} $ is given by 
			$ g_{\cA_2,1,1}(x)\ed \Paren{1+3/{\sqrt{17}}}\Paren{x-5/4+ {\sqrt{17}}/{4}}+1/2 $. 
			For suitable values of $ \delta,m $ we may find $f\in  \cC_{g, \delta, m} $ (whose lower envelope is 
			$ g' $) such that the $ \cA_{2} $ minimizer to $ \hatf $ suffers an error $ > 2.135\OPT_{\cP_{1}}(f) $.}
		\label{fig:1}
	\end{figure}
	It can be shown that $g_{\cA_2,1,1} $ is given by
	\[g_{\cA_2,1,1}(x)\ed \Paren{1+3/{\sqrt{17}}}\Paren{x-5/4+ {\sqrt{17}}/{4}}
	+1/2\ \forall x\in [0,1],\]
	as shown in Figure~\ref{fig:1}.
	
	Suppose $ X^{n}\sim f $ for some $f\in  \cC_{g,\delta,m}  $.
	Recall that $ \hatf $ is the associated empirical distribution.
	Since by construction, all distributions in $ \cC_{g,\delta,m} $
	have nearly identical probability masses in all intervals, and as each 
	distribution is indistinguishable w.p. $ \ge 1-\delta $, it follows that 
	the $\lone{\hatf_{\cA_{2},1,1} - g_{\cA_{2},1,1}}<10/m $ w.p. $ \ge 1-\delta $.
	Suppose we set $ f \in \cC_{g,\delta,m}$  to be a distribution
	with the lower envelope $ g' $ as shown in Figure~\ref{fig:1}. Notice 
	$ \OPT_{\cP_{1}}(f)=1/2 $ whereas its distance to the $\cA_2$ minimizer 
	$ \hatf_{\cA_2,1,1} $ is $ w.p.\ge 1-\delta $,
	\begin{align}
	\nonumber
	\lone{f- \hatf_{\cA_2,1,1}}
	&\overset{}{\ge}\lone{f- g_{\cA_2,1,1}}
	-
	\lone{g_{\cA_2,1,1}- \hatf_{\cA_2,1,1}}
	\\
	\nonumber
	&\overset{}{\ge}\lone{f- g_{\cA_2,1,1}}
	-\frac{10}{m}
	\\
	\nonumber
	&=1.068-\frac{10}{m}\\
	\label{eqn:asdfa}
	&\ge 2.136 \OPT_{\cP_{1}}(f)-\frac{10}{m}
	\end{align}
\end{Proof}
We show that even if one outputs 
an estimate from a larger class consisting of $k>1 $ linear pieces by finding the $ \cA_{2k_1} $ minimizer to $\hatf$ for any $1\le k_1\le k$,
i.e. 
$\hatf_{\cA_{2k_1}, k ,1} \in \cP_{k,1} $,
we still have a lower bound $ >2 $.
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.7]{fig2}
	\caption{Multi-piece envelope for by scaling and shifting $ g $ in Figure~\ref{fig:1} w.r.t.
		$\barI_{4} = ([0,0.25],[0.25,0.5],[0.5,0.75],[0.75,1])$ and $ p_{4}=(1/4\upto 1/4) $. This 
		construction shows an $f\in  \cC_{h, \delta, m} $ such that even a multi piece
		minimizer to $ \hatf $ based on $\cA$ distance suffers an error $ > 2.135\OPT_{\cP_{1}}(f) $.}
	\label{fig:2}
\end{figure}
Suppose for an integer 
$k>0$, $ \barI_{k} = \Paren{I_1\upto I_k}=\Paren{[0,1/k], [1/k,2/k]\upto [(k-1)/k,1]}$ 
is the $k$-equal width partition of $[0,1] $ and  
$ \barp_k $ is the uniform distribution over $ \Delta_{k} $. 
Consider the envelope given by the piecewise 
\[ h = \sum_{i=1}^{k} \mathbbm{1}_{x\in I_{i}} g\Paren{k\Paren{x-\frac{i-1}{k}}}\]
as shown in Figure~\ref{fig:2}.
\begin{Lemma}
	Let $ \hatf $ be the empirical distribution corresponding to $ X^{n}\sim f $.
	For some integer $ k\ge 1 $ and $1\le k_1\le k$ let 
	$ \hatf_{\cA_{2k_1}, k ,1} \in \cP_{k,1}$  be the $ k $-piece linear polynomial that minimizes
	the $ \cA_{2k_1} $ distance to $ \hatf $. Then, there exists a distribution $ f \in \cC_{h,\delta, m}$ such that
	for any $\delta >0$, w.p. $\ge 1-\delta$,
	\[
	\lone{\hatf_{\cA_{2k_1}, k ,1}-f}\ge 2.136 \OPT_{\cP_{1}}(f)-\frac{10}{m}.
	\]
\end{Lemma}
\begin{Proof}
	One of the $ \cA_{2k_1} $ minimizers to $ h$ from the class $ \cP_{t,1} $
	is given by the transformed $ g_{\cA_{2},1,1} $, i.e.,
	\[ h_k \ed \sum_{i=1}^{k} \mathbbm{1}_{x\in I_{i}}  g_{\cA_{2},1,1}\Paren{k\Paren{x-\frac{i-1}{k}}}.\]
	as shown in Figure~\ref{fig:2}. That is
	\[
	h_k  \in \argmin_{q\in\cP_{k,1}}\akk{2k_1}{h} .
	\]
	
	For any distribution in $f\in \cC_{h,\delta,m} $ with lower envelope $ g'=1/2 $,
	as before,
	\[
	\OPT_{\cP_{1}}(f) =\frac12.
	\]
	Thus, along the lines of Equation~\ref{eqn:asdfa}, w.p. $\ge 1-\delta$,
	the $ \ell_{1} $ distance between $ f $ and $\hatf_{\cA_{2k_1}, k ,1} $ may be as large as 
	\begin{align*}
	\lone{f- \hatf_{\cA_{2k_1}, k ,1}}
	&\overset{}{\ge}\lone{f- g_{\cA_2,k,1}}
	-
	\lone{g_{\cA_{2k_1},k,1}- \hatf_{\cA_{2k_1},k,1}}
	\\
	&\overset{}{\ge}\lone{f- g_{\cA_2,k,1}}
	-\frac{10}{m}
	\\
	&=1.068-\frac{10}{m}\\
	&\ge 2.136 \OPT_{\cP_{1}}(f)-\frac{10}{m}
	\end{align*}
\end{Proof}
Thus for any $1\le k_1\le k$,
choosing $\delta\searrow 0$ and $m\nearrow\infty $, we obtain \[\lone{\hatf_{\cA_{2k_1},1,1}}
\ge 2.135 \OPT_{\cP_1}(f)\] with for any arbitrarily high probability $1-\delta$.
In other words ...

On the other hand we show that by a careful modification of the 
$ \cA_{d} $ minimizer we achieve the optimal $ 2\OPT_{\cP_{d}}(f) $ 
for any $ d>0 $.

\ignore{Jul 31 Meeting suggestions\\
	1. Extend $\cA_2$ to general $k$. - Done\\
	2. How to handle cross-validated $\ADLS$?}
\ignore{
	Fix any $ \alpha\ge 1 $, such that $ \alpha\cdot k $ is an integer.
	Consider the class $\cC_{g_{\alpha k},\delta }$ and draw $ X^{n}\sim f $
	according to an $ f\in \cC_{g_{\alpha k},\delta } $ with lower envelope $ q' $.
	
	Recall that $ \hatf $ denotes the resulting empirical distribution.
	The idealized version of the $ \ADLS $ algorithm 
	outputs the $ \alpha k$-piecewise degree-$ 1 $ polynomial 
	$ q_{\IADLS} \in \cP_{\alpha k,1}$ that minimizes the 
	$ \cA_{2k} $ distance to $ \hatf$, namely
	\[
	q_{\ADLS}\ed \argmin_{q\in \cP_{\alpha k,1}}\akk{2k}{\hatf}.
	\]
	%
	Observe that $ q_{\alpha k} $ is one \newbla{(need to write a little more)}
	of the solutions to $\argmin_{q\in \cP_{\alpha k,1}}\akk{2k}{g_{\alpha k}}$ and as
	$ f $ and $ g_{\alpha k} $ are indistinguishable from $ n $ samples $ w.p.\ge 1-\delta $,
	$ q_{\ADLS} $, for any $ n\ge 25 $ suffers w.p $ \ge 1-\delta $ the loss
	\[
	\lone{f-q_{\ADLS} }= 1.068 - \frac{2}{n^2} =2.136 \OPT_{\cP_{\alpha k,1}}(f) - \frac{2}{n^2}
	\overset{(a)}=2.136 \OPT_{\cP_{ k,1}}(f) -  \frac{2}{n^2}
	\overset{(b)}\ge 2.13  \OPT_{\cP_{ k,1}}(f)
	\]
	where $ (a) $ follows since by the choice of $f$, $ \OPT_{\cP_{t,1}}(f) $ is 
	independent of $ t $ for any integer $ t\ge 1 $ and $ (b) $ follows since $ n\ge 30 $
	and $ \OPT_{\cP_{k},1} =1/2$.
}


==> poly.tex <==
\ignore{-.5em}
\section{The Interpolation Routine}
\ignore{-.25em}
\label{sec:black}
This section describes $ \EQ $, which outputs 
an estimate $ \hatf_{I, \EQ} \in \cP_d$ for any queried interval $ I $.

WLOG let $I = [0,1] $. A collection, $ \barn_d = (n_0\upto n_{d+1})$
such that $ 0=n_0\le n_1\le\cdots\le n_d\le n_{d+1}= 1 $
is said to be a node partition of $ [0,1] $.
Let $ \cN_d $ be the set of node partitions and
define $r:\cN_d,\cP_d\rightarrow[1,\infty)$
\begin{equation}
\label{eqn:polyrat}
r(\barn_d,\poly)
\ed
\frac{\int_{0}^1|\poly|}
{\sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}\poly|},
\end{equation}
where $ 0/0\ed 1 $. Notice $r(\barn_d,\poly)\ge 1$ since 
$\int_{0}^1|\poly|\ge \sum_{i=1}^{d+1}|\int_{n_{i-1}}^{n_i}\poly| 
$.
For any $\barn_d\in \cN_d$, let
\[r_d(\barn_d)=\sup_{\poly\in\cP_d}r(\barn_d,h).
\ignore{-1em}
\]

Let $ I_{\barn_d,i} \ed  [n_{i-1},n_i]$, 
$ i\in \{1,\cdots,d+1\} $ so that any 
$ \barn_d \in \cN_{d}$ 
partitions $ [0,1] $ into 
$ \bar{I}_{\barn_d} =(I_{\barn_d,1}\upto I_{\barn_d,d+1})$.
Let $ \hatf_{\barn_d}  \in \cP_{d}$ be the unique 
polynomial whose measure on all $ d+1 $ intervals in $ \barI_{\barn_{d}} $
matches the empirical mass. It is defined as:
\begin{equation}
\label{eqn:areamatch}
\hatf_{\barn_d} \ed h \in \cP_d : 
\forall i \in \{1,\cdots, d+1\} ,
\int_{n_{i-1}}^{n_{i}} h = \hatp_{I_{\barn_d,i}},
\end{equation}
where $ \hatp_{I} $ denotes the empirical 
mass in interval $ I $. 
The estimate $ \hatf_{\barn_d} $ corresponding 
to any choice of $\barn_d\in \cN_d$ has the 
following property.
\begin{Lemma}
\label{lem:ratioconst}
For interval $ I=[0,1]$ with empirical probability 
$ \hatp_I $, any $ \barn_d\in\cN_d $, 
and $ \epsilon>0 $, the estimate $ \hatf_{\barn_d} $~\eqref{eqn:areamatch} is such that
under event $ \cQ_{\epsilon} $,
\begin{align*}
\lone{\hatf_{\barn_d}-f} 
&\le 
\left(1+r_d(\barn_d)\right)
\inf_{\poly \in \cP_d}\lone{\poly-f} \\
&\phantom{\le}
+r_d(\barn_d) \epsilon \sqrt{(d+1)\hatp_I}.
\end{align*}
\end{Lemma}
In Lemma~\ref{lem:zeroish}, we show that for any 
$ \barn_d\in \cN_{d}$, there exists an 
$ r_d(\barn_d)$ achieving $\poly \in \cP_{d} $, 
and that it belongs to a special set, $ \cP_{\barn_d} \subseteq \cP_d$,
\begin{align*}
%\cP_{\barn_d}
%&\ed 
%\Big\{\poly \in \cP_d :
%\forall i\in \{1 \upto d+1\} \setminus \{i_1\},\\
%&\phantom{\ed \Big (}\int_{n_{i-1}}^{n_i}\poly = 0
%\text{ for some }
%i_1\in\{1\upto d+1\} \Big\}.
%change for camera ready
\cP_{\barn_d}
&\ed 
\Big\{\poly \in \cP_d : \exists 
i_1\in\{1\upto d+1\} :\\
&\phantom{\ed \Big (}
\forall i\in \{1 \upto d+1\} \setminus \{i_1\},
\int_{n_{i-1}}^{n_i}\poly = 0\
\Big\}.
\end{align*}
In words, $\cP_{\barn_d}$ is the set of
polynomials that has a non-zero area in at most 
one $ I \in \barI_{\barn_d}$.
\ignore{$ \poly\in\cP_d $ to be considered in when 
finding $ \barn_d \in \cN_d $ with a bounded 
$ r(\barn_d) = \sup_{\poly\in\cP_d}r(\barn_d,h)$.
 Formally,
Lemma~\ref{lem:zeroish} shows that the 
largest ratio over $ \poly \in \cP_d $ is attained 
by some $ \poly \in \cP_{\barn_d}$.}
\begin{Lemma}
\label{lem:zeroish}
For any degree-$d$ and $ \barn_d\in\cN_d $,
\[r_d(\barn_d)=\sup_{\poly\in\cP_d}r(\barn_d,h)
=\max_{\poly\in\cP_{\barn_d}}r(\barn_d,h).\]
\end{Lemma}

Let the smallest $ r_d(\barn_d) $ and the 
attaining $ \barn_d $ (if it exists) be denoted by
\[
r^{\star}_d \ed \inf_{\barn_d\in \cN_d} r_d(\barn_d), \
\barn_d^{\star} 
= \text{arg}\min_{\barn_d\in \cN_d} r_d(\barn_d).\]
Lemma~\ref{lem:optnodes} finds $ r^{\star}_d $
and $ \barn^{\star}_d $ for $ d\le 3 $. Additionally,
for $ 4\le d\le 8 $ it finds $ \barn_d \in \cN_d$ 
such that the corresponding $ r_d(\barn_d) < 2$.
\begin{Lemma}
\label{lem:optnodes}
For $d\le 3 $, there exists a node collection 
$ \barn^{\star}_d $
that achieves $ r^{\star}_d $. These,
and their respective $ r^{\star}_d $ are given by
\begin{center}
\begin{tabular}{ |c|c|c| } 
\hline
$ d $ & $ \barn^{\star}_d $  & $r^{\star}_d$ \\ 
\hline
0 & $ (0,1) $ & $ 1 $ \\
\hline
1 & $ (0,0.5,1) $ & $ 1.25 $ \\
\hline
2 & $ \approx (0, 0.2599, 0.7401, 1) $ & $ \approx 1.42 $ \\ 
\hline
3 & $ \approx(0, 0.1548, 0.5, 0.8452, 1) $& $\approx 1.56 $\\ 
\hline
\end{tabular}
\end{center}
Denoting $\barn^{\star}_2 = (0,\alpha_0,1-\alpha_0, 1)  $, 
and $ \barn^{\star}_3 = (0, \beta_0, 0.5, 1-\beta_0, 1) $,
the exact values of $ \alpha _0 $, $ \beta_0 $, 
are obtained as roots to a degree-$14$ and 
degree-$ 69 $ polynomial that we explicitly provide.
For degrees $ 4\le d\le 8 $, the following 
$ \barn_d\in \cN_d$ and $ r_d(\barn_d) $ 
provide upper bounds on $ r_d^{\star} $.
\begin{center}
\begin{tabular}{ |c|c|c| } 
\hline
$ d $ & $ \barn_d $  & $r_d(\barn_d)$ \\ 
\hline
4 & $ (0, 0.1015, 0.348, 0.652, 0.8985,1)$ & 
$ < 1.675$ \\
\hline
5 & $ ( 0 ,   0.071 ,   0.254 ,   0.5  ,  $ &  \\ 
 & $  0.746,   0.929  ,  1) $ & $ <  1.774 $ \\ 
\hline
6 & $ (0,    0.053,    0.192,    0.390,    $& $ $\\ 
& $   0.610,   0.808,   0.947,    1) $& $ < 1.857 $\\ 
\hline
7 & $ (0, 0.0405   , 0.149 ,  0.310,   0.5,   $ & \\
& $  0.690,    0.851, 0.9595,    1) $ & $ < 1.930 $ \\
\hline
8 & $  (0,    0.032,   0.119,    0.252,    0.414,   $ &  \\
& $  0.586,   0.749,    0.881,   0.968,   1) $ & $ < 1.999 $ \\
\hline
\end{tabular}
\end{center}
\end{Lemma}
For a given interval $ I $ and $ d\le 8 $,
$ \EQ $ first scales and shifts $ I $ to obtain
$ [0,1] $. It then constructs $\hatf_{\barn_d}$ using
the $ \barn_d$ in Lemma~\ref{lem:optnodes}.
The output $\hatf_{I, \EQ}$ is the 
re-scaled-shifted $\hatf_{\barn_d}$.

==> poly69.tex <==
\begingroup
\allowdisplaybreaks
\begin{align*}
&q_3(m)\ed m^{69}
+\frac{2233}{46}m^{68}
+\frac{3394851}{2944}m^{67}
-\frac{26295551}{1472}m^{66}
+\frac{76466381715}{376832}m^{65}
-\frac{1357944230009}{753664}m^{64}\\
&+\frac{627961733592749}{48234496}m^{63}
-\frac{3795194179761079}{48234496}m^{62}
+\frac{1252499739594399621}{3087007744}m^{61}
-\frac{5593584650474780121}{3087007744}m^{60}\\
&+\frac{87541700408454835933}{12348030976}m^{59}
-\frac{9689649149944354300097}{395136991232}m^{58}\\
&+\frac{477481388280085878102175}{6322191859712}m^{57}
-\frac{1316816736336377796401265}{6322191859712}m^{56}\\
&+\frac{104518853645525535726426411}{202310139510784}m^{55}
-\frac{935729957191660731330480575}{809240558043136}m^{54}\\
&+\frac{1894032003216065918256250147}{809240558043136}m^{53}
-\frac{111070063686665905121657252873}{25895697857380352}m^{52}\\
&+\frac{2947966937880382636398337723253}{414331165718085632}m^{51}
-\frac{96053130159826779148472826511}{9007199254740992}m^{50}\\
&+\frac{5957768773291898355944143881565}{414331165718085632}m^{49}
-\frac{28666092800309188568756667723285}{1657324662872342528}m^{48}\\
&+\frac{1936825259310147713677259087614429}{106068778423829921792}m^{47}
-\frac{216663456959495677102483903955187}{13258597302978740224}m^{46}\\
&+\frac{4797689934446961630160031643189779}{424275113695319687168}m^{45}
-\frac{6609917603386978813128872815736861}{1697100454781278748672}m^{44}\\
&-\frac{1831051294952734349349124229564767}{424275113695319687168}m^{43}
+\frac{77448257249275962672807384094624197}{6788401819125114994688}m^{42}\\
&-\frac{3438211574596414864435399648557575571}{217228858212003679830016}m^{41}
+\frac{14691873341415043555417961121466375911}{868915432848014719320064}m^{40}\\
&-\frac{52197058412928213666930233026164438477}{3475661731392058877280256}m^{39}
+\frac{626588406181557032617836659688444683449}{55610587702272942036484096}m^{38}\\
&-\frac{1555525051509188771980730278198868813547}{222442350809091768145936384}m^{37}
+\frac{2911728348738530370986950039544396475929}{889769403236367072583745536}m^{36}\\
&-\frac{415629763783269606797247480824967018319}{618970019642690137449562112}m^{35}
-\frac{21293950227855325096203381076755307029285}{28472620903563746322679857152}m^{34}\\
&+\frac{568117182824342053622453013472967651433283}{455561934457019941162877714432}m^{33}
-\frac{544176155073471826876603760623685652791461}{455561934457019941162877714432}m^{32}\\
&+\frac{26510792231823207111468208052472537291091795}{29155963805249276234424173723648}m^{31}\\
&-\frac{4339252967361049353363803334422356143484711}{7288990951312319058606043430912}m^{30}\\
&+\frac{80732188658524254663695919868749449919506951}{233247710441994209875393389789184}m^{29}\\
&-\frac{21178612540977853104278860543475186392271681}{116623855220997104937696694894592}m^{28}\\
&+\frac{80945977995703186772569013525777965350114711}{932990841767976839501573559156736}m^{27}\\
&-\frac{17702912107607481296775724392303230443070095}{466495420883988419750786779578368}m^{26}\\
&+\frac{113795689628398207709330045266274999410341749}{7463926734143814716012588473253888}m^{25}\\
&-\frac{21034631455622622763256522489198166970683613}{3731963367071907358006294236626944}m^{24}\\
&+\frac{229167532475013797669274973054071362594872031}{119422827746301035456201415572062208}m^{23}\\
&-\frac{17963282649430914596699742603270996080670419}{29855706936575258864050353893015552}m^{22}\\
&+\frac{165857532854257459359651249063603517430127219}{955382621970408283649611324576497664}m^{21}\\
&-\frac{21988393007280087042133518345726499678514793}{477691310985204141824805662288248832}m^{20}\\
&+\frac{2673062517068208952962202401457887091620815}{238845655492602070912402831144124416}m^{19}\\
&-\frac{4753573760248527366859497435267453417384687}{1910765243940816567299222649152995328}m^{18}\\
&+\frac{7698530432612172216840174126420917394335697}{15286121951526532538393781193223962624}m^{17}
-\frac{88254391793832097376072061503233796540539}{955382621970408283649611324576497664}m^{16}\\
&+\frac{466181759012121800363517839555926856292931}{30572243903053065076787562386447925248}m^{15}
-\frac{34314489379863699139383468530966229926169}{15286121951526532538393781193223962624}m^{14}\\
&+\frac{71176987410160907949890583502121075660389}{244577951224424520614300499091583401984}m^{13}
-\frac{3987333962073343668163889901656755306225}{122288975612212260307150249545791700992}m^{12}\\
&+\frac{748668655114740354600745066271570265031}{244577951224424520614300499091583401984}m^{11}
-\frac{110845256761306163606440669442292637027}{489155902448849041228600998183166803968}m^{10}\\
&+\frac{1899176964083859703283044829743633209}{170141183460469231731687303715884105728}m^{9}
-\frac{2073921584792354563737120211683341}{42535295865117307932921825928971026432}m^{8}\\
&-\frac{3440239020182100263379082512521175}{61144487806106130153575124772895850496}m^{7}
+\frac{4264138856148752641548430451717}{664613997892457936451903530140172288}m^{6}\\
&-\frac{3117503551035781118929644883731}{7643060975763266269196890596611981312}m^{5}
+\frac{29037077182037119112722125423}{1910765243940816567299222649152995328}m^{4}\\
&-\frac{46083309361423573178372679}{238845655492602070912402831144124416}m^{3}
-\frac{597811927318403605685541}{59711413873150517728100707786031104}m^{2}\\
&+\frac{30104861649982869480831}{59711413873150517728100707786031104}m
-\frac{105905655782897976459}{14927853468287629432025176946507776}
\end{align*}
\endgroup


==> singlepiece1.tex <==
\section{Single-Piece Polynomials}
\label{sec:singlep}
Our objective is to obtain a min-max $2$-factor approximation for the piecewise $\cP_{t,d}$.
We first achieve this for the single-piece class $\cP_{1,d}$ 
and use the estimator for the general $\cP_{t,d}$.
WLOG suppose $f$ is supported on $[-1,1]$.

We construct our min-max $2$-factor approximation for $\cP_d$ based on two other estimates, namely $g_1$ that approximates $f$ in $\tvv$ distance and $g_2$ that approximates it in $\cA_{d+1}$ distance. Lemma~\ref{lem:splitlem} shows the favorable properties of this estimator.
\begin{Lemma}
\label{lem:splitlem}
Given functions $g_1$ and $g_2$ such that for some $\chi$, $\epsilon>0$,
\[\akk{g_1}{f}\le \chi\]
black-box poly estimator $  \fest_I\in \cP_{d} $ 
that satisfies Definition~\ref{def:tilde}, an interval $ I \subseteq \reals $ and
the integer $k\ge 1$, the transformed estimate $\fspcs{spl}_I$ satisfies
\begin{align*}
\tvi{I}{\fspcs{spl}_{I}}{f}\le & 
\Paren{2+\frac{b(d+1)(c_{1}+1)}{k}}\tvi{I}{f}{\cP_d}+
{\frac{b(d+1)\Paren{c_{2}\akkint{d+1}{I}{\hatf_n -f}+\eta}}{k}}\\
&+\akkint{k}{I}{\hatf_n -f},
\end{align*}
where $ b>0 $ is a numerical constant.
\end{Lemma}



Prior works~\cite{jay17,surf20} that derive min-max $c$-factor bounds for some $c>2$
build on an approximation for $f$ in $\cA_{d+1}$ distance,
leveraging the fact that the $\cA_{d+1}$ distance between two polynomials equals the $\tvv$ distance between them.
% they derive polynomial min-max $c$-factor estimators for some $c>2$. 
We also use this technique, albeit indirectly, by using the above type of estimators as a black-box, formally defined below.
%  which includes the estimates considered for $t=1$ in~\cite{jay17,surf20}.

\begin{Decaf}
\label{def:tilde}
For any $ c>0$, given any real function $g$, $\fspcs{poly}(g)$
is said to be a black-box poly estimator if for some universal 
constant $\chi>0$,
% $\fspcs{poly}(g(\epsilon)) \in \cP_d$ is said to be a 
% {black-box poly estimator} for $ \cP_{d} $ if
% for any additive approximation $\eta>0$,
\begin{align*}
\tv{\fspcs{poly}(g)}{f}
\le c\cdot \tv{f}{\cP_d} +\chi\cdot \akk{d+1}{f-g}.
\end{align*}
\end{Decaf}



% This is accomplished by a routine that transforms 
% a $c$-factor polynomial approximate estimator for the class $ \cP_{d} $ with its optimal $\epsilon_n=\cO(\cR_n(\cP_d))$. 

% Given a function $g$ that approximates $f$ in $\cA_d$ distance, we derive its approximation $\tvv$ distance.
% The previous approaches gave a method to derive $3$ a factor .. we refine these techniques... 


% We transform the min-max $c$-factor approximate estimators
% for $\cP_d$ considered in~\cite{jay17,surf20}.

Notice that a natural choice of $g = \hatf_n$. With this choice it straightforward to observe that $\fspcs{poly}$ is also a min-max $c$ factor approximation for $\cP_d$, as from the 
VC inequality (Lemma~\ref{lem:vc}) it follows that $\EE\akk{d+1}{f-g}=\cO(\sqrt{(d+1)/n})$.

WLOG consider the interval $I=[-1,1]$ and let $\fspcs{poly}$ denote the black-box poly estimate on $[-1,1]$.
Our main idea is based on the observation if there exists a
function $g$ that has the same area as $f$ in $I$, and
% that any distribution $\fspcs{distr}$ 
% which does not intersect 
which does not intersect with the degree-$d$
polynomial closest to $q$, then
% the
% $\tv{q}{\cP_d}$ achieving polynomial, $q^*\in \cP_d$, 
$\tv{g}{f}\le 2\tv{q}{\cP_d}$. 
It is easy to show that from Definition~\ref{def:tilde} that $\fspcs{poly}$ must have nearly the probability mass of $f$ in $I$. However  the $\fspcs{poly}\in \cP_d$ may intersect up to $d$ times with $p$ in general.
We transform $\fspcs{poly}$ using the masses of $g$ corresponding to a carefully constructed partition of $[-1,1]$ to 
diminish the contribution to the $\tvv$ distance that arises from these intersections.

Let $\barJ_k$ denote this partition of $[-1,1]$, consisting of $\le k$ intervals.
The guiding principle behind the choice of $\barJ_k$ is to bound the $\tvv$
distance between any degree-d polynomial $p\in \cP_d$
and its histogram on $\barJ_k$, $\barp_{\barJ_k}$. Observe that if $W(I)$ denotes the width of interval $I$,
\begin{equation}
\label{eqn:324}
\tvi{I}{p}{\bar{p}_I}
\le W(I)\cdot \int_I |p'(t)|dt.
\end{equation}
Lemma~\ref{lem:poly} bounds the quantity on the RHS, $\int_I |p'(t)|dt$ in terms of the $ \ell_{1} $ norm of $p$.
\begin{Lemma}
\label{lem:poly}
For any degree-$ d $ polynomial $p\in \cP_{d}$ and $x\in(-1, 1)$,
\[
\int_{-x}^{x}|p'(t)|\, dt
%
\,\le\,
\frac{28(d+1)}{\sqrt{1-x^2}}
%
% \,\lesssim\,
% \frac{d}{\sqrt{1-x^2}}
%
\int_{-1}^1|p(t)|\, dt.
\]
\end{Lemma}
% \[
% |f(x)|\sqrt{1-x^2}
% \le
% d
% \int_ |f(t)| dt
% \]
%
The proof uses the Bernstein and Markov Brothers' inequality 
and may be found in Appendix~\ref{sec:appen3}.
\textcolor{purple}{Ask Yi to add some details and intuition}.

Suppose we set $\barJ_k$ to be the uniform partition of $[-1,1]$
with $k$ intervals.
Notice that using Lemma~\ref{lem:poly} along with Equation~\eqref{eqn:324}, the 
$\tvv$ distance between the $p$ and its histogram on this partition diminishes as $k\rightarrow\infty$ in all regions of the partition, except along the extremes of $[-1,1]$.
% However Lemma~\ref{lem:poly} is loose for regions that are close to the extrema of $[-1,1]$.
Our approach modifies this uniform partition such that the interval widths decrease nearly geometrically towards the extremes so as to bound the $\tvv$ distance also in these regions.

Let $ \barJ_k $ denote the partition used in $ \SPLIT $.
For $i\ge 1$ define the region 
$I_i\ed  [-(1-1/2^{i}), -(1-1/2^{i-1})]\cup[1-1/2^{i-1}, 1-1/2^i]$.
Partition $I_i$ into $l (d+1)/2^{i/4}$ sub-intervals of equal width denoted by $\barI_i$. 
Thus each interval is of width $1/2^{i}\cdot 2^{i/4}/(l(d+1)) = 1/(2^{3i/4}\cdot l(d+1))$.
% Let $\barI_{i} $ denote this partition of $ I_{i} $.
For an integer $ m\ge 1 $ collect $ {\cup_{i=1}^m\barI_i} $
and let 
 $E_{m}\ed [-1,1]\setminus \Paren{\cup_{i=1}^m\barI_i}$
 denote the two terminal intervals.
By construction, observe that the width of the terminal region 
$ |E_{m}|\le 2/2^{m} $.
Define 
\begin{equation}
\label{eqn:l}
l\ed (2^{1/4}-1)k/(d+1),
\end{equation}
and for an $\epsilon>0$, let $m(\epsilon)\ed \log_2(l(d+1)^2/\epsilon)$ so that $|E_{m(\epsilon)}|\le 2
\epsilon/(l(d+1)^2)$. Define \[\barJ_k(\epsilon) \ed  \cup_{i=1}^{m(\epsilon)}\barI_i \cup E_{m(\epsilon)}.\]

Lemma~\ref{lem:polyhist} bounds the $ \ell_{1} $ difference between 
any polynomial $ p\in \cP_{d} $ and its histogram on $ \barJ_k(\epsilon) $ denoted by 
$ \bar{p}_{\barJ_k(\epsilon)} $.
Recall 
% that $\barp_{\barJ}$ refers to the histogram of $p$ on the partition $\barJ$ and 
that $\loneint{I}{p}$ refers to the $\ell_1$ norm of $p$ in interval $I\subseteq \reals$.
\begin{Lemma}
\label{lem:polyhist}
For some constant $b\le ...$, for all $ p \in \cP_{d} $ and $ k\ge 0 $, 
the partition $ \barJ_k(\epsilon) $ with $\le k$ intervals 
%the histogram of $ p $ under the 
satisfies
\[
\tvi{[-1,1]}{p}{\barp_{\barJ_k(\epsilon)}} \le b\cdot \frac{\loneint{[-1,1]}{p}}{2k}+\epsilon/4.\]
\end{Lemma}

%For a given $0\le c_1\le 1/2$ and $l\ge 0$, let $k(c_1,l)$
% %denote the 
% %number of intervals in $ \barJ $. 
% We use
% Lemma~\ref{lem:polyhist} in bounding the $\ell_1$ distance between the optimal polynomial $q^*_I$ and $\fest_I$. The bias component of the error 
% in approximating $p$ with its histogram 
% $\barJ$. However, in the application of Lemma~\ref{lem:polyhist} that we consider
% the area under $ p $ in each interval in $ \barJ_k $ is unknown. This results in an 
% additional error that roughly takes the form
% $\akkint{k(c_1,l)}{I}{\hatf_n -f }$. In order to upper bound this term, we would also 
% like $ \barJ $ to have as few intervals as possible. 
We now show that the number of intervals in the partition $\barJ_k(\epsilon)$ is upper bounded by $k$, for all values of $\epsilon>0$.
\[
|\barJ_k(\epsilon)| = \sum_{i=1}^{m(\epsilon)} |\barI_i| 
= \sum_{i=1}^{m(\epsilon)}  \frac{l(d+1)}{2^{i/4}} 
\le 
\frac{l(d+1)}{2^{1/4}}
\cdot \frac{1}{1-2^{-1/4}}
=\frac{l(d+1)}{2^{1/4}-1}\le k,
\]
where the last step follows from the definition of $ l $ in Equation~\ref{eqn:l}. As the number of intervals for any $\epsilon$ 
is upper bounded by $k$, for simplicity we use 
$\barJ_k=\lim_{\epsilon\rightarrow 0}\barJ_k(\epsilon)$ to obtain the best possible accuracy in Lemma~\ref{lem:polyhist}.

%For simplicity choose $ c_{1} = 1/4 $,
%so that $ \barJ(c_{1},) $ consists of $\le  12l(d+1)$ intervals. 

As the number of intervals in $\barJ_k$
is upper bounded by $k$, we may use the empirical $\hatf_n$
to estimate the probability mass of $f$ in each of these intervals.
The masses are used to apply the following transformation to the black-box polynomial estimate (defined in Definition~\ref{def:tilde}).
\begin{Definition}
\label{def:polytranslate}
Given a partition $\barI$  of an interval $ I \subseteq \reals$, 
a collection of masses 
$\bar{m}_{\barI}\ed (m_I\in \reals, \ I\in\barI)$, and a function $q\in I$, we define the translation of $ q $ w.r.t. $ \barm_{\barI}$ as
\[
q_{\bar{m}_{\barI}, \barI}(x)  \ed \sum_{I\in \barI}\mathbbm{1}_{x\in I}
( q(x)+m_{I}).\]
% \text{ where for any interval $ J \subseteq \reals$, } 
% {m}_J \ed \int_{J} h(x)- q(x)dx.
\end{Definition}
Definition~\ref{def:polytranslate} along with Lemma~\ref{lem:polyhist}
implies Corollary~\ref{cor:polyhist} that bounds the difference between 
polynomials that are `translated' w.r.t. the same set of  masses.
\begin{Corollary}
\label{cor:polyhist}
Given polynomials $ p,q\in \cP_{d} $, an interval $ I \subseteq \reals $, and an integer $ k\ge 1 $,
for any collection of masses $\barm_{k} $ defined on $\barJ(I)_k$,
the $\tvv$ distance between their translations w.r.t. $\barm_k$,
\[
\tvi{I}{p_{\barm_{k},\barJ_k}}{q_{\barm_k,\barJ_k}}
\le 
\newbla{b}\frac{\tvi{I}{p}{q}}{l}
.
\]
\end{Corollary}
Corollary~\ref{cor:polyhist} implies that by translation along the the $\cO(k)$ interval partition $\barJ_k$, the $\tvv$ distance between any two polynomials may be decreased by a multiplicative factor of $\cO(1/l)=\cO((d+1)/k)$.
We use this result in proving the main Lemma of this section below.
\newbla{Update proof of Corollary~\ref{cor:polyhist} (and possibly Lemma~\ref{lem:splitlem}) with the new notation.}

Recall that $\fspcs{poly}$ denotes the black-box estimate that we use as a subroutine (ref. 
Definition~\ref{def:tilde}). Let $\bar{p}_{\barJ_k}$ denote the collection of empirical probability masses on intervals in $\barJ_k$.
Using the construction described above, the $ \SPLIT $ output estimate given by
\[
\fspcs{spl}_I \ed \fspcs{poly}_{\bar{p}_{\barJ_k}, \barJ_k}.
\]
In other words $ \fspcs{spl} $ is obtained via adding a constant to 
$ \fspcs{poly}$ in
each interval in $\barJ_k$ to match its mass with the empirical mass in that interval.
% \newbla{consider removing} $ \SPLIT $ is summarized in Algorithm~\ref{alg:SPLIT}. 
Lemma~\ref{lem:splitlem} shows that $\fspcs{spl}_I$ is a min-max $2$-factor approximate estimator for $\cP_d$.
% \begin{algorithm}[h]
% 	\caption{$ \SPLIT $}
% 	\label{alg:SPLIT}
% 	\begin{algorithmic}
% 		\STATE {\bfseries Input:} $ X^{n} $, $ d $, $ I $, $ \tilde{q} $, $ k $
% 		\STATE {\bfseries Output:} $ \barJ_k, \tilde{q}_{\hatf, \barJ_k}$
% 	\end{algorithmic}
% \end{algorithm}


\subsection{Polynomial rate optimal estimators for $ \cP_{d} $}
\label{sec:adlslala}
We now describe in more detail the black-box estimators (ref. Definition~\ref{def:tilde}) in existing literature that we consider.
The work~\cite{surf20} describes an estimator $ \fspcs{surf}_I $ for
any interval $ I\subseteq $ that is given by matching probability masses 
to $ \hatf_n $ on a specially constructed, pre-defined partition of $ I $ with $d+1$ intervals. $\fspcs{surf})_I $ achieves the following as stated in Lemma 6~\cite{surf20}.
\begin{Lemma}
Consider an interval $ I $ with $ n_{I} $ samples. The $ \fspcs{surf}_I $ estimate 
is computable in $ \cO(n_{I}(d+1)^\omega) $ time and satisfies
\[
\tvi{I}{ \fspcs{surf}_I }{f}\le c_{d}\cdot \tvi{I}{f}{\cP_{d}}+\akkint{d+1}{I}{\hatf_n-f},
\]
where $ c_{d} $ is a constant that depends on $ d $
and $ \omega< 3 $ is the matrix multiplication/inversion constant.
\end{Lemma}
In~\cite{surf20} it is also shown that $ c_{d} $ is a small 
value for most practical degrees of interest. E.g. $ c_{d}<3 $ for the degrees $ 0\le d\le 8 $ that are used to learn $ f $ that is Unimodal, Log-concave
or Gaussian mixture.

If it is desired to use larger degrees, at the expense of 
a greater computation time, 
the work~\cite{jay17} describes the construction of a projection oracle 
based estimator, $ \fspcs{adls}_I( \eta) $ for any $\eta>0$.
Lemma~\ref{lem:proj} from~\cite{jay17} provides the following guarantee for this estimator.

\newbla{Probably Lemma~\ref{lem:proj} not needed, only Corollary~\ref{cor:adlsis42} required. Part of final clean up.}
\begin{Lemma}~\cite{jay17}
\label{lem:proj}
Consider an interval $ I\subseteq \reals $, $ \eta > 0$ with $n_I$ samples. Then the estimate $\fspcs{adls} $ satisfies
\[
\akkint{d+1}{I}{\fspcs{adls}_I(\eta)-\hatf_n}
\le \min_{q\in \cP_d}\akkint{d+1}{I}{q-\hatf_n} + \eta
\]
in time
\[
\cO\Paren{\Paren{d^{3}\log \log \frac1n +n_{I}d^{2}+d^{\omega +2}}\log^{2}\frac1{\eta}},
\]
where $ n_{I}$ refers to the number of samples in interval $ I $
and $ \omega<3 $ is the matrix multiplication constant.
\end{Lemma}
By a straightforward application of triangle inequality on top of Lemma~\ref{lem:proj}, we show below that $\fspcs{adls}_I( \eta)$ satisfies Definition~\ref{def:tilde}.
\begin{Lemma}
\label{cor:adlsis42}
For any $ \eta>0 $, $ \fspcs{adls}_I(\eta) $ is 
computable in $\cO(n_Id^{w+2}\log^2(1/\eta))$ time and satisfies 
\[
\tvi{I}{\fspcs{adls}_I(\eta)}{f}
\le 3\cdot \tvi{I}{f}{\cP_d}
+2\akkint{d+1}{I}{\hatf_n-\hatf_n} + \eta.
\]
\end{Lemma}	


%Using $ \tilde{q}_{I} = \tilde{q}_{\cA_{d+1}}$,
%the the estimate output by $ \SPLIT $, $ \hatq_{I} $,
%achieves a 2-factor approximate estimator for 
%$ \cP_{d} $ along with the optimal
% $ \epsilon_{n} = \cO(\akkint{d+1}{I}{\hatf-f}) $. This 
%is stated in the following corollary:
%\begin{Corollary}
%	Given the $ \eta $ approximate
%	$ \cA_{d+1} $ minimizer to $ \hatf_n $ in $ I $, $  \tilde{q}_{\cA_{d+1}} $ 
%	returned by $ \PROJ(\hatf, I, \eta) $,
%	and numbers $l\ge 0$, $1/2>c_1\ge 0$,
%	$ \SPLIT $ returns the piecewise $ \hatq_{I} $ such that
%	\[
%	\loneint{I}{\hatq_{I}-f}\le  \Paren{2+\frac{56}{l(1-2^{c_1-1/2})}}\tvi{I}{f}{\cP_d}+
%	{\frac{28\Paren{2\akkint{d+1}{I}{\hatf_n -f}+\eta}}{l(1-2^{c_1-1/2})}}+\akkint{k}{I}{\hatf_n -f},
%	\]
%	where we recall that $k\ed {l(d+1)}/{(2^{c_1}-1)}$ is a constant 
%	multiple of $ d+1 $.
%\end{Corollary}


